GS-NBV: a Geometry-based, Semantics-aware Viewpoint Planning Algorithm for Avocado Harvesting under Occlusions

Efficient identification of picking points is critical for automated fruit harvesting. Avocados present unique challenges owing to their irregular shape, weight, and less-structured growing environments, which require specific viewpoints for successful harvesting. We propose a geometry-based, semantics-aware viewpoint-planning algorithm to address these challenges. The planning process involves three key steps: viewpoint sampling, evaluation, and execution. Starting from a partially occluded view, the system first detects the fruit, then leverages geometric information to constrain the viewpoint search space to a 1D circle, and uniformly samples four points to balance the efficiency and exploration. A new picking score metric is introduced to evaluate the viewpoint suitability and guide the camera to the next-best view. We validate our method through simulation against two state-of-the-art algorithms. Results show a 100% success rate in two case studies with significant occlusions, demonstrating the efficiency and robustness of our approach. Our code is available at https://github.com/lineojcd/GSNBV

==> sections/0_0_abstract.tex <==
\begin{abstract}
% For automated fruit harvesting, identifying the picking point is essential. 
% Unlike other fruits, picking avocados require specific viewpoints due to their unique harvesting challenges and highly unstructured growing environments.
Efficient picking point identification is critical for automated fruit harvesting. 
Avocados present unique challenges due to their irregular shape, weight, and less-structured growing environments, requiring specific viewpoints for successful harvesting. 
In this work, we propose a geometry-based, semantics-aware viewpoint planning algorithm to address these challenges.
% To automated fruit harvesting, the fruit picking point needs to be found first.
% Unlike other fruits, picking avocados requires specific viewpoints. 
% Additionally, the highly unstructured growing environment of avocados makes it more challenging.
% In this work, we propose a novel geometry-based, semantics-aware viewpoint planning algorithm to address these issues. 
% We introduce the picking score metric to evaluate selected viewpoints and constrain the viewpoint search space to a 1D picking ring to improve planning efficiency.
% \textcolor{red}{We first detect fruit; constrain the viewpoint search space to a 1D picking ring to improve planning efficiency.  then introduce the picking score metric to evaluate selected viewpoints and }
The planning process 
iterates through three key steps: viewpoint sampling, evaluation and execution.
Starting from a partially occluded view, the system first detects the fruit, then leverages geometric information to constrain the viewpoint search space to 1D, uniformly sampling four points to enhance efficiency. A novel picking score metric is introduced to evaluate viewpoint suitability and guide the camera to the next best informative view.
We validate our method through comparative simulation experiments against two state-of-the-art algorithms. Results show a 100\% success rate in two challenging simulated environments, demonstrating the efficiency and robustness of our approach. The code will be publicly available on GitHub upon publication.
% is achieved through multiple iterations.Each iteration consists of three key steps: randomly generatingcandidate views, predicting the ideal perspective using a scorefunction, and guiding the robotic arm to change the viewpoint.
% Our approach first detects the fruit from a partially visible view. Then we 
% fruit  from  avocado and peduncle, constrains the viewpoint search space to 1D  and uniform adaptively sampled 4 viewpoints space to enhance planning efficiency, then we introduce a novel picking score metric to evaluate viewpoint suitability.
% Finally, to validate the effectiveness and robustness of the planner, we conducted comparative experiments on Kinova Jaco2 arm with other state-of-the-art methods in two challenging simulated environments. 
% Finally, we conducted comparative experiments on Kinova Jaco2 arm with two state-of-the-art methods. The results demonstrate a 100\% success rate in two challenging simulated environments, verifying the efficiency and robustness of our planning algorithm.
% in-lab settings with a single attempt, and field trials further verify the system’s robustness and efficiency in more challenging real-world environments
% The results verify the practicality of our algorithm.
% The code will be publicly available on GitHub upon publication.
% The code will be made publicly available on github.com
% (upon publication, if accepted).

% % occlusion problem and find out the avocado picking point.
% 
\end{abstract}


==> sections/1_1_intro_picking_point.tex <==
% \subsection{Picking point}
% Fruits such as apple, orange and etc. have smooth surface and a rather uniform spherical shape. 
% In this case, their picking points are distributed almost over the entire fruit surface.
Fruits such as apple, orange and etc. have smooth surfaces and a rather uniform spherical shape. The picking points are almost distributed over the entire fruit surface.
This property, sole requirement of end effector coming in direct contact with the fruit, simplifies both mechanical complexity (enabling vacuum-powered suction cups commonly used~\cite{hemming2014robot, bontsema2014crops, hayashi2010evaluation}) and algorithmic complexity (enabling the sufficiency of solely the fruit 3D position information to complete the harvesting task~\cite{li2022occluded}). 
Some fruits such as cherry tomatoes, blueberry and etc. are small, delicate and light weighted. They can be picked up by wrapping the pneumatically-actuated deformable fingers
% (soft gripper) 
around the fruits~\cite{navas2024soft}. 
In this case, their picking points are still distributed almost over the entire fruit surface.
Some fruits such as grape~\cite{jiang2022development}, pepper~\cite{lehnert2017autonomous} and etc. can be picked up by employing a scissor-like mechanism to cut off the fruit peduncle.  In this case, their picking points are on the fruit peduncle or flower stalk. Similar cases include strawberry~\cite{yu2019fruit}, litchi~\cite{zhuang2019computer} and etc. 
Generally, in the above cases, obtaining 3D position of the fruit or peduncle is sufficient to complete the harvesting task.
\begin{figure}[!t]
% \vspace{4pt}
    \centering
    % \includegraphics[trim={1cm 8cm 2cm 0cm},clip,width=0.45\textwidth]{figs/first_page_pic.png}
    \includegraphics[width=0.45\textwidth]{figs/demo_pic_nbv_pipeline.png}
    \vspace{-2 pt}
    \caption{Illustration of GS-NBV. The scene is represented using a Semantic Octomap: the background is teal, the avocado is red, and a green cube marks the pre-defined region-of-interest (ROI). The ground truth picking ring is magenta. Grey arrows indicate previously selected viewpoints, magenta arrows show candidate viewpoints in the Queue, and blue arrows highlight the selected viewpoints from the current iteration. Small yellow arrows are valid viewpoints sampled on the estimated picking ring.
    The robotic arm is depicted in black at the current viewpoint and in transparent at the next-best viewpoint (shown as a red arrow).
    \textcolor{red}{Combine Fig1 ad3, make a photorealistic, Octomap representation, initial view and fina view on One image and add legend to avoid lenth text}
    }
    \label{fig:algo_demo}
    \vspace{-22pt}
\end{figure}

However, for fruits like avocados, obtaining this information 
% 3D position of the fruit 
% only obtaining this information 
alone is insufficient for
% cannot complete 
automated harvesting.
Avocados are heavier, less uniformly shaped, and have a bumpy surface, making them unsuitable for vacuum or soft-based end effectors. 
% On one hand, avocados are much heavier, have a less uniform shape (spheroid), and their surface is irregularly textured
% with bumps; hence it cannot be picked up by vacuum-based or soft-based end effectors. 
% On the other hand, avocados 
Additionally, they must be cleanly detached from the peduncle 
to facilitate
% for 
efficient packaging and transportation purpose. 
The peduncle-cutting method is also unsuitable, as the remaining peduncle can cause damage to other avocados and accelerate decay~\cite{zhou2024design}.
% \textcolor{green}{On another hand,  peduncle-cutting method is also not proper because avocado peduncle will harden when cut, it is important to remove it before packaging as it can otherwise damage other avocados in the container (e.g., cause punctures) and lead to faster decay of all products in the same container. To optimize the harvesting process, our goal is to thus remove the avocado from its peduncle cleanly~\cite{zhou2024design}.}
Due to these unique characteristics, avocado can only be effectively picked up from some specific viewpoints: canonical view (CV) and front view (FV)~\cite{zhou2024design} (Fig.~\ref{fig:avocado_env_ring}). 
% Consequently, obtaining merely the 3D position is insufficient; acquiring the 6D pose of the avocado is essential.
% \textcolor{red}{Consequently, acquiring the 6D pose of the avocado is essential for automatic harvesting.}
% Therefore, acquiring the 6D pose of the avocado is essential for automatic harvesting.
Therefore, acquiring the avocado’s 6D pose is crucial for successful automated harvesting.
% This requirement poses significant challenges to the development of automated picking algorithms.

==> sections/1_2_intro_occlusion.tex <==
% \subsection{Occlusion}

In addition to identifying the picking points, another common challenge in automated harvesting is occlusion issue.
% another common issue in automated harvesting is occlusion: the occlusions from leaves usually make obtaining fruit pose difficult.
% due to the occlusion caused by leaves, it may not be possible to directly estimate the fruit pose from the current view. 
In recent years,
% With advancements in computer vision, 
many efforts have been made to address fruit pose estimation under occlusion.
The main methods include picking point prediction~\cite{yu2019fruit}, fruit shape completion~\cite{marangoz2022fruit, gong2022robotic, pan2023panoptic, yao2024safe} and viewpoint planning.
The first two methods mainly make predictions on the current view through prior knowledge or learning fashion~\cite{gong2022robotic, li2024single}. 
These works for regular shaped fruit, but not well-suited for avocados (avocado has more than 500 cultivars~\cite{de2020convolutional}, 
% different cultivars can vary drastically in their size and volume
varying drastically in their shape, size and volume~\cite{mokria2022volume}).
In contrast, viewpoint planning approach iteratively determines the most informative sensor viewpoints, making it a promising solution for reducing uncertainty in object or space perception.

Several studies have employed next-best view (NBV) planning to tackle occlusion issue. Zaenker et al.~\cite{zaenker2021viewpoint} constructed a voxel map of plants with labeled regions of interest (ROIs), then used viewpoint sampling to select the most informative views around the ROI. 
They later introduced a graph network built on feasible view poses~\cite{zaenker2023graph} to account for robot motion constraints. 
Additionally, multi-camera systems~\cite{zaenker2021combining, lehnert20193d} have also been explored for local and global viewpoint planning, allowing for local occlusion avoidance while covering large areas, though with limited generalizability across different platforms. 
These sampling-based NBV methods depend on computationally expensive ray-casting algorithms to evaluate viewpoints. 
To mitigate this, Menon et al.~\cite{menon2023nbv} introduced viewpoint dissimilarity to reduce the search space for more efficient selection of useful, dissimilar viewpoints. 
Zeng et al.~\cite{zeng2022deep} proposed a deep reinforcement learning-based NBV framework using encoded 3D observation maps, though it struggles with generalization, even in simulation. 
Akshay et al.~\cite{burusa2024gradient} introduced a gradient-based optimization approach that eliminates viewpoint sampling, significantly improving efficiency. However, this method is prone to getting stuck in local maxima, greatly reducing its reliability.

Although these methods partially address occlusion, they primarily focus on environment exploration and fruit coverage rather than harvesting in heavily occluded settings, where picking points are initially fully obscured. 
Tao et al.~\cite{yi2024view} introduced the Spatial Coverage Rate metric (SC-NBVP) to identify grape picking points by constructing a voxel map only around the stem region. 
Their method, tailored for structured vineyard environments, achieves rapid planning (under two seconds) even with extensive viewpoints sampling.

\begin{figure}[!t]
\vspace{6pt}
    \centering
    % \vspace{-6pt}
    \begin{subfigure}[b]{0.260\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/avo_env_small_brighter.jpg}
        % \caption{}
        \label{fig:avo_env}
    \end{subfigure}
    \hspace{0.0005\textwidth} 
    \begin{subfigure}[b]{0.210\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/fruit_coord_picking_ring_1_brighter2.jpg}
        % \caption{}
        \label{fig:picking_ring}
    \end{subfigure}
    \vspace{-28pt}
    \caption{
    Left: Avocado growing environment. Right: Fruit coordinate system and picking ring.}
    \label{fig:avocado_env_ring}
    \vspace{-22pt}
\end{figure}
However, unlike fruits grown in controlled greenhouse environments (Fig.~\ref{fig:avocado_env_ring}), avocados are grown in unstructured orchards, making existing solutions difficult to generalize effectively.
To address these challenges, we propose a novel geometry-based, semantics-aware viewpoint planning algorithm 
% \textcolor{red}{built on top of the Semantic Octomap framework~\cite{burusa2024gradient}, (can removed)}
built on the Semantic OctoMap framework~\cite{burusa2024gradient}
for automated avocado harvesting in heavily occluded environments.
To the best of our knowledge, this is the first reported automated picking algorithm specifically targeting avocados.
Our key contributions are:

==> sections/1_2_intro_occlusion_ori.tex <==
% \subsection{Occlusion}

In addition to identifying the picking points, another common challenge in automated harvesting is occlusion issue.
% another common issue in automated harvesting is occlusion: the occlusions from leaves usually make obtaining fruit pose difficult.
% due to the occlusion caused by leaves, it may not be possible to directly estimate the fruit pose from the current view. 
In recent years,
% With advancements in computer vision, 
many efforts have been made to address fruit pose estimation under occlusion.
The main methods include picking point prediction~\cite{yu2019fruit}, fruit shape completion~\cite{marangoz2022fruit, gong2022robotic, pan2023panoptic, yao2024safe} and viewpoint planning.
The first two methods mainly make predictions on the current view through prior knowledge or learning fashion~\cite{gong2022robotic, li2024single}. 
These works for regular shaped fruit, but not well-suited for avocados (avocado has more than 500 cultivars~\cite{de2020convolutional}, 
% different cultivars can vary drastically in their size and volume
varying drastically in their shape, size and volume~\cite{mokria2022volume}).
By contrast, the latter approach iteratively determines the most informative viewpoint for a sensor, which appears to be a promising solution for reducing uncertainty about the observed 
object or space. 
% object~\cite{yi2024view} or space~\cite{zeng2022deep}. 
% At present, many viewpoint planning algorithms are specifically designed for fruits grown in greenhouse environments~\cite{menon2023nbv}. However, avocados are not grown in greenhouses but in highly unstructured environments~\cite{vasconez2022workload}. The severe occlusion in such settings presents further challenges for automated picking algorithms.
% Currently, many existing picking algorithms are specifically designed for fruits cultivated in controlled greenhouse environments~\cite{menon2023nbv, pan2023panoptic}. 

Currently, most existing picking algorithms are specifically designed for fruits cultivated in controlled greenhouse environments~\cite{menon2023nbv, pan2023panoptic}. 
In contrast, avocados are grown in highly unstructured settings, where severe occlusion poses significant challenges to current automated picking algorithms. To date, no effective and robust method has been designed to automate avocado harvesting in such environments.
% While some existing research focuses on human-robot collaborative strategies to improve harvesting efficiency for avocados~\cite{vasconez2022workload}, no significant work has been conducted on fully automated algorithms.
% Except for the picking point difference, another major difference compared to other fruits is that avocados does not have greenhouse planting~\cite{pan2023panoptic}. It grows in a highly unstructured environment.
% The heavy occlusion makes it difficult to view the entire fruit body from a single view and to accurately estimate its pose. 

% ----Planning algo and NBV --- goes here

% Therefore in this work, we developed a XXX implemented by XXX 
% Yet, there is still a lack of automated robotic picking up algorithms designed for avocado harvesting to date. 
% In this paper, we focus on design an automated picking algorithm to harvest avocado.

\begin{figure}[!t]
    \centering
    % \vspace{-6pt}
    \begin{subfigure}[b]{0.260\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/avo_env_small_brighter.jpg}
        % \caption{}
        \label{fig:avo_env}
    \end{subfigure}
    \hspace{0.0005\textwidth} 
    \begin{subfigure}[b]{0.210\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/fruit_coord_picking_ring_1_brighter2.jpg}
        % \caption{}
        \label{fig:picking_ring}
    \end{subfigure}
    \vspace{-26pt}
    \caption{
    Avocado growing environment (left). Fruit coordinate system and picking ring (right).}
    \label{fig:avocado_env_ring}
    \vspace{-16pt}
\end{figure}


% The difference, however, is that avocados grow in unstructured, highly occluded environment (Fig.~\ref{fig:avo-env}).
% structured cultivation has not yet become popular, which 
% Therefore the growth direction of fruits is not completely vertical downward. 
% Meanwhile, it is also quite challenging to localize the fruit from the bottom view due to occlusion issues in the wild growing condition. 

% To this end, we developed a rigid finger-based with a two-stage rotational motion end effector and also defined some specific viewpoints: canonical view (CV) and front view (FV) as picking point (Fig.~\ref{fig:picking_ring}) for the end effector. Based on previous findings, in this work, we define the picking points on a ring surrounding the fruit on the plane spanned by CV and FV, and we call it the picking ring (Fig.~\ref{fig:picking_ring}). 

% \begin{figure}[!t]
% % \begin{figure}[hpb]
%     % \vspace{-12pt}
%     \centering
%     \includegraphics[width=0.45\textwidth]{figs/avo_fv_cv_view_paper_s.png}
%     \vspace{-14pt}
%     \caption{Fruit coordinate system
%     % and viewpoints for the avocado
%     % \textcolor{red}{TODO: say more like red means easier, blue means harder and etc}
%     }
%     \label{fig:fruit_coor_system}
%     \vspace{-22pt}
% \end{figure}

==> sections/2_0_related_work.tex <==
\section{Related work 
}
In agriculture, the occlusion issues have consistently posed significant challenges to the automation of fruit harvesting. 

% Several works used the next-best view (NBV) planning approach to address the occlusion issue.
% Zaenker et al.~\cite{zaenker2021viewpoint} constructed a voxel map of plants with labeled regions of interest (ROIs), then sampled candidate viewpoints around the ROI and selected the viewpoint with highest information gain as the next-best view. In their subsequent work~\cite{zaenker2023graph}, they constructed a graph network of feasible view poses to account for robot motion constraints.

% In~\cite{zaenker2021combining}, they integrated a specialized multi-camera array from~\cite{lehnert20193d} into their system, combining local and gradient-based global viewpoint planning. This allows for local occlusion avoidance while covering large areas, but the approach is hard to generalize to other platforms. The above sampling-based methods generate a set of candidate viewpoints and use a computationally expensive ray-casting algorithm to evaluate their utility. To reduce costs, Menon et al.~\cite{menon2023nbv} introduced viewpoint dissimilarity to narrow the sampling space and find the next best view through missing surfaces of the fruit shape. However, this method only applies to regularly shaped fruits, such as orange, pepper and etc.
% X. Zeng et al.~\cite{zeng2022deep} converted the octomap into an encoded 3D observation map and used it in a deep reinforcement learning network to determine the next best view. However, this approach is difficult to generalize, even in simulated environments.
% Akshay et al.~\cite{burusa2024gradient} proposed a gradient-based optimisation algorithm by using a differentiable utility function to avoid the drawbacks of sampling-based approaches: the camera moves directly to local maximized viewpoint without sampling. 
% While this approach significantly reduces computational costs, it is prone to getting stuck in local maxima, which greatly diminishes the system's reliability.

% Although these methods partially address occlusion, they primarily focus on environment exploration and improved fruit coverage rather than harvesting in heavily occluded settings, where picking points are initially fully obscured.
% Tao et al.~\cite{yi2024view} introduced the Spatial Coverage Rate metric (SC-NBVP) to 
% identify grape picking points by constructing a voxel map around the stem region.
% Benefiting from the structured growth of grapes, their planning process takes less than two seconds even with extensive viewpoints sampling.

% Our approach shares similarities with SC-NBVP, as we also detect the peduncle for avocado harvesting.
% Additionally, we introduce a picking score metric to evaluate selected viewpoints. 
% To the best of our knowledge, this is the first automated avocado harvesting algorithm designed for heavy occlusion conditions.


==> sections/2_0_related_work_ori.tex <==
\section{Related work 
% \textcolor{red}{Refine later}
}
% \textcolor{red}{Technical detail goes here}
% Viewpoint planning often use in task xxx and xxx and xxx. 
% Active vision is a well-researched topic, it can be used in plant phenotyping, fruit size estimation~\cite{zaenker2021viewpoint} and mapping crop fields.  However, 
In agriculture, the occlusion issues have consistently posed significant challenges to the automation of fruit harvesting. 

Several works used the next-best view (NBV) planning approach to address the occlusion issue.
% In agro-food sector, occlusion issue have consistently posed significant challenges to the automation of fruit harvesting. Several works use the next-best view (NBV) planning approach to address the occlusion issue: 
% Several works use the next-best view (NBV) planning approach to address the occlusion issue: 
Zaenker et al.~\cite{zaenker2021viewpoint} constructed a voxel map of plants with labeled regions of interest (ROIs), then sampled candidate viewpoints around the ROI and selected the viewpoint with highest information gain as the next-best view. In their subsequent work~\cite{zaenker2023graph}, they constructed a graph network of feasible view poses to account for robot motion constraints.
\begin{figure}[!t]
    \centering
    % \vspace{-6pt}
    \begin{subfigure}[b]{0.2414\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/paper_sim_scene_trim640.png}
        % \caption{Fruit contour and surrounding curve}
        \label{fig:cont_sur_curve}
    \end{subfigure}
    % \hspace{0.0005\textwidth} 
    \hspace{-5pt} 
    \begin{subfigure}[b]{0.2410\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/paper_curve_3_trim.png}
        % \caption{Simulation setup}
        \label{fig:sim_env_setup}
    \end{subfigure}
    \vspace{-26pt}
    \caption{Left: In the Gazebo simulation environment, the RealSense D435i camera is mounted at the center of the Jaco2 arm's end-effector.
    % replacing the original finger gripper. 
    The avocado is partially visible within the camera's current field of view. 
    Right: The contour (magenta) and surrounding curve (blue) are extracted from the avocado mask, predicted by the YOLOv8 model~\cite{Jocher_Ultralytics_YOLO_2023}.
    % , and displayed in magenta and blue, respectively. 
    \textcolor{red}{will merge with Fig 1 later}
    }
    \label{fig:curve_sim_fruit}
    \vspace{-26pt}
\end{figure}
In~\cite{zaenker2021combining}, they integrated a specialized multi-camera array from~\cite{lehnert20193d} into their system, combining local and gradient-based global viewpoint planning. This allows for local occlusion avoidance while covering large areas, but the approach is hard to generalize to other platforms. The above sampling-based methods generate a set of candidate viewpoints and use a computationally expensive ray-casting algorithm to evaluate their utility. To reduce costs, Menon et al.~\cite{menon2023nbv} introduced viewpoint dissimilarity to narrow the sampling space and find the next best view through missing surfaces of the fruit shape. However, this method only applies to regularly shaped fruits, such as orange, pepper and etc.
X. Zeng et al.~\cite{zeng2022deep} converted the octomap into an encoded 3D observation map and used it in a deep reinforcement learning network to determine the next best view. However, this approach is difficult to generalize, even in simulated environments.
Akshay et al.~\cite{burusa2024gradient} proposed a gradient-based optimisation algorithm by using a differentiable utility function to avoid the drawbacks of sampling-based approaches: the camera moves directly to local maximized viewpoint without sampling. 
% Although this method greatly reduces the computational cost, it is prone to getting stuck in local maxima.
While this approach significantly reduces computational costs, it is prone to getting stuck in local maxima, which greatly diminishes the system's reliability.
% While building a GPU-compatible voxel map greatly reduces computational costs, this method is prone to getting stuck in local maxima.

% Although the above methods can solve the occlusion problem to a certain extent, they mainly focus on environment exploration and better fruit coverage not on precise fruit pose estimation in a local heavy occlusion setting.
% Although the above methods can solve the occlusion problem to a certain extent, they mainly focus on environment exploration and better fruit coverage not on how the fruit is harvested in a local heavy occlusion setting where the fruit picking points are initially fully occluded.
Although these methods partially address occlusion, they primarily focus on environment exploration and improved fruit coverage rather than harvesting in heavily occluded settings, where picking points are initially fully obscured.
Tao et al.~\cite{yi2024view} introduced the Spatial Coverage Rate metric (SC-NBVP) to 
identify grape picking points by constructing a voxel map around the stem region.
% identify the grape picking point on the stem. Thanks to the grape's structured growing environment, they construct the voxel map only around the stem region. 
% Despite extensive viewpoint sampling, the planning process takes less than two seconds.
Benefiting from the structured growth of grapes, their planning process takes less than two seconds even with extensive viewpoints sampling.
% Our method shares similarity with SC-NBVP: we also need to detect the peduncle for avocado harvesting. 
Our approach shares similarities with SC-NBVP, as we also detect the peduncle for avocado harvesting.
% However, the difference is we sample a few viewpoints based on geometry and semantic information to avoid computational cost. Furthermore, we also introduced a metric called picking score to evaluate the selected views.
Additionally, we introduce a picking score metric to evaluate selected viewpoints. 
% To the best of our knowledge, this is the first viewpoint planning algorithm for automated avocado harvesting under heavy occlusion.
% To the best of our knowledge, this is the first reported automated avocado harvesting algorithm developed for heavy occlusion conditions.
To the best of our knowledge, this is the first automated avocado harvesting algorithm designed for heavy occlusion conditions.
% this is the first automated avocado harvesting algorithm developed for heavy occlusion conditions.

% Dec-MCTS~\cite{sukkar2019multi} did xxx, limitation is xxx
% Introducing the category: global planning, local planning\\
% Need to introduce GNBV, SCNBVP, Maybe providing tables of NBV: RVP and RVP familiy}
% also describe local vs gblocal NBV task
% \textcolor{blue}{

% \textcolor{blue}{-----The whole section is under writting now-----}
% \\
% Another major difference compared to other fruits is that avocados grow in a highly unstructured environment. The heavy occlusion makes it difficult to view the entire fruit body from a single view and to accurately estimate its pose. With advancements in computer vision, several efforts have been made to address fruit pose estimation under occlusion ~\cite{yu2019fruit, lehnert20193d}.
% Among these, active vision is a promising solution.
 
% % List some works in 2D based (what did they do, how did they do, what problem do they solve and still left) . or just say it is hard to solve avocado picking point issue in 2d. Active vision is a promising solution.
% Check the NBV paper for this part writing.  then start comparing NBV algos.
% (providing tables NBV: RVP and RVP familiy)
% also describe local vs gblocal NBV task

% \textcolor{blue}{
% However, the above-mentioned works do not mention how the harvesting is achieved when the fruit picking point is partially or fully occluded}

% -1.~\cite{yu2019fruit, lehnert20193d} Fruit detection for strawberry harvesting robot in non-structuralenvironment based on Mask-RCNN  
% Chinese researchers Yu, Y. et al., (2019) used a Mask R-CNN instance segmentation network modelto recognize overlapping strawberries and apples, respectively. They can determine notonly categories but also individuals. Since some ripe green tomatoes are similar in colorto branches and leaves, shaded by branches and leaves, or overlapped by other tomatoes,accurate detection and localization of these tomatoes is difficult.
% My summary:
% Use get fruit segmentation mask by Mask-RCNN, calculate the fruit axis and find the picking point on this axis approximately 13–20 mm away from the fruit mask.
% solve multi-fruit adhesion , overlapping, and the occlusion of stems and leaves. \\

% -2. ~\cite{zhuang2019computer}
% Computer vision-based localisation of pickingpoints for automatic litchi harvesting applications towards natural scenarios

% find picking point through tradition computer vision algo. and tackle the illumination changes that  affect picking point.

% ~\cite{li2020detection}
% Detection of Fruit-Bearing Branches and Localization of Litchi Clusters for Vision-Based Harvesting Robots
% mainly involved thefollowing steps:(a) Semantic segmentation based on Deeplabv3 to segmentthe fruits, branches, and background in RGB images.(b) Morphological process analysis to obtain informationabout the fertile branches.(c) Revised DBSCAN clustering-based branch extractionand optimal clustering parameter analysis. (d) Spatial straight line fitting and localization of fertilebranches.

% In this study, one image includedone litchi cluster, and the stem was not occluded. 

% solve this problem: detect and locate small fruit-bearing branches in a large environment where one captured image contains mul-tiple litchi strings to be picked. 

 % The growth of litchi clusters on a tree is typically randomand irregular, so it is difficult to simultaneously detect and locate the fruit-bearing branches of multiple litchi bunches in one image, which presents a major challenge to vision-basedharvesting robots that are intended to perform continuousoperations under natural environments. 

% However, to date,no such research has been reported in this regard. 
% In arecent study [37], the authors considered prioritizing robotic grasping of stacked fruit clusters with small stalks on the basis of RGB-D images, which is one of the most relevant studies addressing this challenge. 

% Therefore, we have alsoattempted to research this issue. Inspired by object segmenta-tion based on deep convolutional neural networks and fruit 3Dlocalization methods, this study aims to develop a combinedalgorithm to detect and locate small fruit-bearing branches in a large environment where one captured image contains mul-tiple litchi strings to be picked. 
% \\
% Other similar work including XX and XX and XXX
% \\
% List 3D based 
% \\
% The problem is occlusion


==> sections/3_0_problem_formulation_and_setup.tex <==
\section{Problem description and set up}
% \subsection{Preliminary Definitions}
% \vspace{-3pt}
% To pick up avocados in the presence of occlusions, we first need to establish some definitions.
\begin{figure}[!t]
\vspace{6pt}
    \centering
    % \vspace{-6pt}
    \begin{subfigure}[b]{0.2414\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/paper_sim_scene_trim640.png}
        % \caption{Fruit contour and surrounding curve}
        \label{fig:cont_sur_curve}
    \end{subfigure}
    % \hspace{0.0005\textwidth} 
    \hspace{-5pt} 
    \begin{subfigure}[b]{0.2410\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/paper_curve_3_trim.png}
        % \caption{Simulation setup}
        \label{fig:sim_env_setup}
    \end{subfigure}
    \vspace{-26pt}
    \caption{Left: Gazebo simulation environment.
    % replacing the original finger gripper. 
    The avocado is partially visible within the camera's current field of view. 
    Right: The contour (magenta) and surrounding curve (blue) are extracted from the avocado mask, predicted by the YOLOv8 model~\cite{Jocher_Ultralytics_YOLO_2023}.
    % , and displayed in magenta and blue, respectively. 
    %\textcolor{red}{will merge with Fig 1 later}
    }
    \label{fig:curve_sim_fruit}
    \vspace{-22pt}
\end{figure}
We used a potted avocado tree model to simulate its growing environment in the real world. 
An RGB-D camera (Intel Realsense D435i) is mounted on the end-effector of a 6-DOF Kinova Jaco2 arm to explore the environment (Fig.~\ref{fig:curve_sim_fruit}). Some preliminary definitions are established beforehand:
% To pick up avocados in the presence of occlusions, we first establish some preliminary definitions.
\label{section:picking_ring}
\begin{enumerate}
    \item \textit{Picking ring:}  
    Circumferential 1D region in the x-y plane defining optimal avocado picking points.% (Fig.~\ref{fig:avocado_env_ring}).
    \item \textit{Discoverability ($s_{dis}$):} Binary metric indicating Object-of-Interest (OOI) visibility; %When both are visible in a scene and their pixels overlap or the nearest distance is below a pixel threshold (set to 5), 
    $s_{dis}=1$, if fruit and peduncle are both visible and overlapping or within a 5-pixel proximity; %\textit{fully discoverable};  
    $s_{dis}=0$ otherwise.
    \item \textit{Contour and surrounding curve (C, R):} Fruit contour (C) and dilated surrounding curve (R).
    %The contour and surrounding curve of the detected fruit in the current view, denoted by magenta and blue color (Fig.~\ref{fig:curve_sim_fruit})
    %\textcolor{red}{Need to mention that surrounding is dilated by Contour curve}.
    \item \textit{Occlusion rate ($s_{occ}$):} Proportion of $R$ with depth less than $d_{f\text{min}} + 0.06$m, where $d_{fmin}$ is the minimum fruit depth, i.e. %The percentage of pixels on the surrounding curve that has depth value less than the sum of the minimum depth value of the fruit pixels and a certain offset value (set as a fixed value 0.06m, which is larger than the majority avocados radius~\cite{zhou2024design}. The equation is 
    $s_{occ} = {\sum_{p \in R} \mathbb{I}\{d_p < (d_{f\text{min}} + d_{\text{offset}})\}}/|R|$. %If the fruit is not occluded at all, the occlusion rate is close to 0.
    \item \textit{Picking score ($s_{pick}$):} 
    %A continuous value distributed between 0 and 1, used to evaluate the 
    Success rate of fruit picking from the current view defined as     % in the current scene. 
    $s_{pick} = s_{dis} * (1-s_{occ})$. A fruit is considered pickable if $s_{pick}>0.9$. %is greater than a threshold (set to 0.9), we say the fruit is \textit{pickable} and then conduct harvest operation. 
% \vspace{-6pt}
\end{enumerate}
% \subsection{Simulation setup} 
% \subsection{Problem Description}
% \vspace{-3pt}
% We downloaded an open avocado model from GrabCAD~\cite{grabcad} and a potted avocado tree model from Sketchfab~\cite{sketchfab} 
% The potted plant is placed within the workspace of the robotic arm, and the fruit is discoverable in the initial camera view.
% is fruit discoverable.
% \vspace{-4pt}
% \subsection{Problem description}

Given a potted avocado plant placed within the arm workspace $V\subset\mathbb{R}^3$, the region $V_{\text{ooc}} \subseteq V$represents the area occupied by the plant, whereas $V_{\text{ooi}} \subseteq V_{\text{ooc}}$ 
% indicates the location of the fruit. 
represents a region that encompasses the avocado, depicted as a green cuboid (Fig.~\ref{fig:algo_demo}).
Initially, $V_{\text{ooi}}$ and $V_{\text{ooc}}$ are unknown. The planner will plan the arm moving within the free space $V_{\text{free}} \subseteq V$. Our task is to explore the region $V_{\text{ooi}}$, starting from a pose where the fruit is partially visible and finally place the camera in a pose that is pickable ($s_{pick} > 0.9$).


==> sections/3_0_problem_formulation_and_setup_ori.tex <==
\section{Problem description and set up}
% \subsection{Preliminary Definitions}
% \vspace{-3pt}
% To pick up avocados in the presence of occlusions, we first need to establish some definitions.
\begin{figure}[!t]
    \centering
    % \vspace{-6pt}
    \begin{subfigure}[b]{0.2414\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/paper_sim_scene_trim640.png}
        % \caption{Fruit contour and surrounding curve}
        \label{fig:cont_sur_curve}
    \end{subfigure}
    % \hspace{0.0005\textwidth} 
    \hspace{-5pt} 
    \begin{subfigure}[b]{0.2410\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/paper_curve_3_trim.png}
        % \caption{Simulation setup}
        \label{fig:sim_env_setup}
    \end{subfigure}
    \vspace{-26pt}
    \caption{Left: In the Gazebo simulation environment, the RealSense D435i camera is mounted at the center of the Jaco2 arm's end-effector.
    % replacing the original finger gripper. 
    The avocado is partially visible within the camera's current field of view. 
    Right: The contour (magenta) and surrounding curve (blue) are extracted from the avocado mask, predicted by the YOLOv8 model~\cite{Jocher_Ultralytics_YOLO_2023}.
    % , and displayed in magenta and blue, respectively. 
    \textcolor{red}{will merge with Fig 1 later}
    }
    \label{fig:curve_sim_fruit}
    \vspace{-22pt}
\end{figure}
We used a potted avocado tree model to simulate its growing environment in the real world. 
An RGB-D camera (Intel Realsense D435i) is mounted on the end-effector of a 6-DOF Kinova Jaco2 arm to explore the environment (Fig.~\ref{fig:curve_sim_fruit}). Some preliminary definitions are established beforehand:
% To pick up avocados in the presence of occlusions, we first establish some preliminary definitions.
\label{section:picking_ring}
\begin{enumerate}
    \item \textit{Picking ring:}  
    The ring-like 1D area surrounds the fruit on the x-y plane, with the ideal picking points for avocados located along the ring (Fig.~\ref{fig:avocado_env_ring}).
    \item \textit{Objects-of-interest (OOI):} In this work, we set fruit and peduncle as OOI, the rest part of the plant is classified as background. If the fruit and peduncle are both visible in a scene, we call it an OOI pair.
    \item \textit{Attachable:} If the detected OOI pair has overlapping pixels or the distance between the nearest pixels of the OOI pair is less than a threshold (we set to 5 pixels here), we say the detected OOI pairs are attachable.
    \item \textit{Discoverable ($s_{dis}$):} 
    % A discrete value \{0, 1\} that indicates the visibility of OOIs.
    % To address the issue that elastic energy stored in peduncle hindering efficient harvesting, we present bimanual harvester in~\cite{liu2024vision}. Therefore,
    $s_{dis}$ is a discrete value \{0, 1\} that indicates the visibility of OOIs. When the fruit and peduncle are both visible, $s_{dis}=1$ and we call it \textit{fully discoverable}. Otherwise, $s_{dis}=0$ indicates only the fruit is visible.
    % To perform harvesting, the fruit and peduncle must be both visible, $s_{dis}=0$. If they are both partially visible and attachable, we call it \textit{fully discoverable}, $s_{dis}=1$. 
    % and the value is 1. 
    % If none of the OOIs are visible, we call it \textit{non-discoverable}, $s_{dis}=-1$ 
    % \item \textit{Discoverable ($s_{dis}$):} A discrete value \{-1, 0, 1\} that indicates the visibility of OOIs.
    % To perform harvesting, either the fruit or the peduncle must be at least partially visible, $s_{dis}=0$. If they are both partially visible and attachable, we call it \textit{fully discoverable}, $s_{dis}=1$. 
    % % and the value is 1. 
    % If none of the OOIs are visible, we call it \textit{non-discoverable}, $s_{dis}=-1$ 
    % and the value is -1. when fully discoverable, otherwise 0.    
    \item \textit{Contour and surrounding curve (C, R):} The contour and surrounding curve of the detected fruit in the current view, denoted by magenta and blue color (Fig.~\ref{fig:curve_sim_fruit}).
    % \item \textit{Surrounding curve (R):} The surrounding curve of the detected fruit in the current view, denoted by blue color(Fig.~\ref{fig:cont_sur_curve}).
    % \item \textit{Contour curve (C):} The contour of the detected fruit in the current view, denoted by red color (Fig.~\ref{fig:cont_sur_curve}).
    % \item \textit{Surrounding curve (R):} The surrounding curve of the detected fruit in the current view, denoted by blue color(Fig.~\ref{fig:cont_sur_curve}).
    % \item \textit{Max and Min fruit depth \( (d_{fmax}, d_{fmin}) \):} The maximum and minimum depth value of the fruit detected in the current view. 
    % To avoid sensor noise and reduce computation, we only search for the maximum depth value from the contour curve.
    \item \textit{Occlusion rate ($s_{occ}$):} The percentage of pixels on the surrounding curve that has depth value less than the sum of the minimum depth value of the fruit pixels and a certain offset value (set as a fixed value 0.06m, which is larger than the majority avocados radius~\cite{zhou2024design}. The equation is $s_{occ} = {\sum_{p \in R} \mathbb{I}\{d_p < (d_{f\text{min}} + d_{\text{offset}})\}}/|R|$. If the fruit is not occluded at all, the occlusion rate is close to 0.
    \item \textit{Picking score ($s_{pick}$):} A continuous value distributed between 0 and 1, used to evaluate the success rate of fruit picking from the current view.
    % in the current scene. 
    The equation is $s_{pick} = s_{dis} * (1-s_{occ})$. When the $s_{pick}$ is greater than a threshold (set to 0.9), we say the fruit is \textit{pickable} and then conduct harvest operation. 
    % \item \textit{Pickable:} A discrete variable \{0, 1\} is used to decide whether to execute the final picking action. When the picking score is greater than a threshold (set to 0.8 in this paper), we consider the fruit is pickable, and the value is 1; otherwise, it is 0.
% \vspace{-6pt}
\end{enumerate}
% \subsection{Simulation setup} 
% \subsection{Problem Description}
% \vspace{-3pt}
% We downloaded an open avocado model from GrabCAD~\cite{grabcad} and a potted avocado tree model from Sketchfab~\cite{sketchfab} 

The potted plant is placed within the workspace of the robotic arm, and the fruit is discoverable in the initial camera view.
% is fruit discoverable.
% \vspace{-4pt}
% \subsection{Problem description}
Given a potted avocado plant placed within the arm workspace $V\subset\mathbb{R}^3$, the region $V_{\text{ooc}} \subseteq V$represents the area occupied by the plant, whereas $V_{\text{ooi}} \subseteq V_{\text{ooc}}$ 
% indicates the location of the fruit. 
represents a region that encompasses the avocado, depicted as a green cuboid (Fig.~\ref{fig:algo_demo}).
Initially, $V_{\text{ooi}}$ and $V_{\text{ooc}}$ are unknown. The planner will plan the arm moving within the free space $V_{\text{free}} \subseteq V$. Our task is to explore the region $V_{\text{ooi}}$, starting from a pose where the fruit is partially visible and finally place the camera in a pose that is pickable ($s_{pick} > 0.9$).


==> sections/4_0_method.tex <==
\section{Method Proposed}
% \subsection{System Overview}
\begin{figure}[!t]
% \begin{figure}[hpb]
    % \vspace{-12pt}
    \centering
    \includegraphics[width=0.45\textwidth]{figs/sys_overview_color_4.png}
    \vspace{-2pt}
    \caption{System overview: the green, yellow, and purple colors represent the sensing, 3D representation and viewpoint planning module respectively. \textcolor{red}{will merge with Fig 3 later}}
    \label{fig:system_overview}
    \vspace{-20pt}
\end{figure}
The automated picking system is an iterative process consisting of three main modules: sensing, 3D representation, and viewpoint planning. Fig~\ref{fig:system_overview} shows an overview of our system framework.
\subsection{Sensing}
% \begin{figure}[!t]
%     \centering
%     % \begin{subfigure}[b]{0.15\textwidth}
%     %     \centering
%     %     \includegraphics[width=\textwidth]{figs/input_rgb_1.png}
%     %     \caption{}
%     %     \label{fig:rgb_input}
%     % \end{subfigure}
%     \vspace{-13pt} 
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/paper_avo_peduncle2_new.png}
%         % \caption{}
%         \label{fig:rgb_img_seg}
%     \end{subfigure}
%     \hspace{-5pt}
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figs/paper_avo_peduncle_octomap_crop.png}
%         % \caption{}
%         \label{fig:semantic_octomap_fake}
%     \end{subfigure}
%     \vspace{-26pt}
%     \caption{Left: Anotated Img Right: Semantic Octomap 
%     % \textcolor{red}{Will made the image better later}
%     }
%     \label{fig:fruit_sensing}
%     \vspace{-20pt}
% \end{figure}
\subsubsection{Object Detection}
% To plan viewpoints to find the picking points that around fruits, 
The first step is to detect the fruit from the scene. We used YOLOv8~\cite{Jocher_Ultralytics_YOLO_2023}  to perform instance segmentation on the input 
% color 
image sequences from a RGB-D camera and generate a segmented image with class label, confidence score and mask.
% The annotated images are also published onto a ROS topic for user visualization .
% (Fig.~\ref{fig:fruit_sensing}). 
The network is fine-tuned to detect avocado and peduncle using a custom dataset of 108 RGB images (640x640 pixels), collected from the simulated environment. 
% (Fig.~\ref{fig:rgb_input}).
A K-fold cross-validation (K=108) strategy is used for training.
% The network undergoes training through cross-validation, employing a K-fold (K=108) strategy to split the dataset.
Since our work is simulation-based, factors like illumination, surface reflections and other sample variations are not considered. 
% Since our work is conducted in a simulated environment, we do not need to consider factors such as illumination, surface reflections, and other sample variations. 
Therefore, the actual data we collected is only 36 images. The other images are generated by built-in data augmentation strategies such as applying rotation, changing color saturation, and adding up 2\% noise.
% \subsubsection{Depth Map Filtering} 
% The D435i sensor utilizes stereo vision technology to generate depth information~\cite{d435i}. However, due to ill-matching or out-of-range measurements issues, the resulting depth map contains some invalid values. 
% To address this, we set a near and far clipping planes at 0.03 m and 0.72 m respectively to clamp the depth values.
\subsubsection{Fruit Pose Estimation and Update} 
\label{subsubsection:fruit_position}
Fruit pose consists of position and axis, defined as $\boldsymbol{f} = \{\boldsymbol{f}_{pos}, \boldsymbol{f}_{axis}\}$, where $\boldsymbol{f}_{pos} \in V_{\text{ooi}} 
% and $\boldsymbol{f}_{axis}
$. 
The detected fruit and its depth values were then converted into point cloud in the world frame.
To mitigate ill-matching and out-of-range measurement issues inherent in the D435i 
sensor,
% sensor’s stereo vision technology~\cite{d435i}, 
we applied depth clipping at 0.03 m (near) and 0.72 m (far) to refine the depth map.
The fruit position is estimated as the mean of the point cloud, with outliers filtered using a one-standard-deviation threshold to mitigate sensor noise.
% The fruit position is 
% % estimated 
% calculated by
% % calculating 
% the mean of its corresponding 
% % points.
% point cloud.
% To mitigate the effect of sensor noise, we only use the points that fall within one standard deviation of the fruit depth value,
% % initial mean, 
% as the sensor noise was the primary source of error in this work. 
The fruit axis is simply calculated as the norm of the difference between the highest and lowest fruit points. Due to occlusion, 
the estimated axis may deviate significantly from the z-axis.
% the angle between the estimated fruit axis and the z-axis can vary significantly. 
Here, we bound the angle to a maximum of 30 degrees, as the avocado axis is unlikely to deviate significantly from the z-axis due to the influence of gravity. When the new observations were made, fruit position and axis are updated by the equation:
$\boldsymbol{f} = \boldsymbol{f}_{t-1} + k * (\boldsymbol{f}_{t} - \boldsymbol{f}_{t-1})$, which computes a weighted average of the fruit pose across multiple observations.
% In this equation，
We set $k$ to 0.7
to assign greater weight to the most recent estimates, as newer observations bring better views and are more likely to result in a better
% more accurate 
pose estimation.
\subsubsection{Obstacle Points Estimation and Update} 
\label{subsubsection:obstacle_points}The pixels on the surrounding curve that has 
$d_p < d_{f\text{min}}$, $d_p \in R$ are obstacle points. 
% By extracting the corresponding depth values from the depth map and converting the points from image pixel frame to world frame, we obtain the obstacle points $P_{occ}$. 
By extracting the corresponding depth values and converting it from image pixel frame to world frame, we obtained the obstacle points $P_{occ}$. 
% \textcolor{red}{In each observation, we only keep the leftmost and rightmost obstacle points into a list for efficiency.}  
When the new observations were made, we append new obstacle points into the same list.
% In each observation, we only keep the leftmost and right most obstacle points for our algorithm.
% \subsubsection{Compute Occlusion Rate and Picking Score} 
\subsubsection{Compute the picking score} 
Each time, when the camera was moved to a new viewpoint, the picking score is computed to determine fruit pickability. 
The planning process concludes once a pickable viewpoint is found.
% the picking status of the current view. 
% Once the fruit is pickable, the planning process conclude.

\subsection{Semantic OctoMap}
Our method is built on the Semantic OctoMap framework~\cite{burusa2024gradient}.
The semantic OctoMap is a 4D voxel grid $\mathcal{M} \in \mathbb{R}^{W \times H \times D \times C}
$ of width \textit{W}, height \textit{H}, depth \textit{D}, and channels \textit{C}.
To fully represent the potted avocado plant, we set \textit{W}, \textit{H}, \textit{D} as (0.42, 0.45, 0.84) m.
Each voxel 
% has a size of 0.003m and 
has 4 channels: occupancy probability, semantic class label, semantic probability, and ROI indicator.  We define a cuboid centered at the initial estimated fruit position (shown in green in Fig.~\ref{fig:algo_demo}), with dimensions of (0.2, 0.2, 0.3) m in width, length and height, marked as regions of interest (ROI). Although the initial estimated fruit position is not exact, the ROI is sufficient large to encompass the entire fruit and peduncle.
Our objective is to explore this ROI to accurately estimate the fruit pose and identify viewpoints that is pickable. 
The semantic class labels include \textit{background}, \textit{avocado} and \textit{peduncle}, 
while all other settings follow~\cite{burusa2024gradient}.
% while all other settings, such as occupancy probability, semantic class probability 
% % and OctoMap update
% follow~\cite{burusa2024gradient}.

The Semantic OctoMap is updated by 
Raycasting algorithm~\cite{hornung2013octomap}.
Upon acquiring new observations, the occupancy probability
% $p_o(x)$ 
% for these voxels 
was updated through addition operation on 
% their 
log-odds value, and then converted back to probability.
The semantic class
% $c_s(x)$ and semantic probability 
% $p_s(x)$ 
and probability 
were updated using a max-fusion method from~\cite{semantic_slam}. 
% It has two cases: when the new class label matches the current class label, $p_s$ is set as the average of the new and current values. 
% When the new class label differs from the current class label, the class label with higher semantic probability is used for update and $p_s$ is updated to this higher semantic probability multiplying a penalty coefficient (here we adopted 0.9, the same setting as in~\cite{burusa2023efficient}). 
% If the two class labels are different, $p_s$ is updated with the class label that has higher semantic probability and multiplying a penalty coefficient (here we adopted 0.9, the same setting as in~\cite{burusa2023efficient}).
% This dynamic updating process ensures that the voxel map accurately reflects changes in environmental observations as the planning progresses.
% However, 
The ROI did not change.
% indicator 
% remains unchanged.
% , as it will be used for comparison with other methods.
\input{sections/4_1_nbv_algo}


==> sections/4_1_nbv_algo.tex <==
\subsection{Viewpoint Planning: GS-NBV}
The viewpoint planning algorithm is an iterative method consisting of 2 main steps: viewpoint sampling and evaluation.
% viewpoint evaluation. 
% Considering the distribution of avocado picking points, we proposed a \textbf{G}eometry-based, \textbf{S}emantics-aware \textbf{N}ext-\textbf{B}est \textbf{V}iew planning algorithm, termed GS-NBV. 
In this section, we first define the utility score to evaluate viewpoints, then elaborate our algorithm (Alg.~\ref{alg:mynbv}). 
% \vspace{-6pt}
\subsubsection{Viewpoint Utility Score}
\label{subsubsection:vp_eva}
The score consists of two parts: the expected semantic information gain 
% $G_{\text{sem}}(\boldsymbol{v})$ 
and 
% the 
motion cost.
% $G_{\text{sem}}(\boldsymbol{v})$
$G_{\text{sem}}(\boldsymbol{v}) = \sum_{x \in (X_v \cap V_{\text{ooi}})} T(x)I_{\text{sem}}(x)$,
 quantifies the total expected semantic information gain from a given viewpoint $\boldsymbol{v}$~\cite{burusa2024gradient}. 
% The equation is 
% the expected semantic information gain estimated
% $G_{\text{sem}}(\boldsymbol{v}) = \sum_{x \in (X_v \cap V_{\text{ooi}})} T(x)I_{\text{sem}}(x)$.
Here 
$X_v$ is the set of all voxels within the field of view, given viewpoint $\boldsymbol{v}$. 
$V_{ooi}$ is the set of ROI voxels. $T(x)$ is an indicator function which determines the visibility from a viewpoint $\boldsymbol{v}$ to a voxel $x$.
In~\cite{burusa2024gradient}, $ T(x)$ measures the accumulated transmittance along the ray up to point $x$, estimating the probability that the ray remains unobstructed. This allows for occluded semantic voxels within the field of view to still enhance information gain.
In our approach, $ T(x)$ is conceptualized differently: 
% Conversely, in our case, 
the invisible semantic voxels do not contribute to information gain. If no semantic voxels are directly visible in the given viewpoint,  $G_{\text{sem}}(\boldsymbol{v})$ equals zero. 
This adjustment enhances the quality of candidate viewpoints by strictly enforcing visibility constraints.
The semantic information $I_{\text{sem}}(x)$ follows~\cite{burusa2024gradient}, which 
measures uncertainty using Shannon’s entropy.
% used to measure uncertainty and calculated through Shannon's entropy. 
% Unlike~\cite{burusa2024gradient}, we exclude the background class, focusing solely on OOIs rather than the surrounding space.
The difference is we exclude background class as our focus is exploring OOIs, rather than the surrounding space. 
% The semantic information $I_{\text{sem}}(x)$ of a voxel $x$ within the field of view of the viewpoint is used to measure uncertainty and calculated through Shannon's entropy: $I_{\text{sem}}(x) = -p_s(x) \log_2(p_s(x)) - (1 - p_s(x)) \log_2(1 - p_s(x))
% $, where $p_s(x)$ is the 
% semantic probability
% that the voxel $x$ belonged to a certain non-background semantic class, ie. $c_s(x)\neq 1$ (our focus is on exploring objects of interest, rather than the surrounding space).
% In addition to expected semantic information gain, 
The Euclidean distance d from the current viewpoint was 
% also 
used when selecting the next best view. 
The final utility score is given by: 
$ U_{\text{sem}}(\boldsymbol{v})= G_{\text{sem}}(\boldsymbol{v}) \times e^{-\lambda d}
$, where 
% $d$ is the Euclidean distance between the current viewpoint and the next potential viewpoint and 
$\lambda$ controls the motion cost penalty. 
Unlike global planning methods that favor adjacent positions, our local planning prioritizes exploration. Moving to a distant viewpoint on the picking ring enhances target coverage. Thus, we set $\lambda = -1$ to encourage larger movements.
% While most methods prioritize adjacent positions, in our local environment planning, motion cost is less critical. Moving to a distant position on the picking ring can intuitively enhance exploration of the target's surroundings. Hence, we set $\lambda$ to -1 to encourage distant movement.
% \vspace{-20pt}
\vspace{-10pt}
\begin{algorithm}
\caption{GS-NBV planning}
\label{alg:mynbv}
\begin{algorithmic}[1]
\Statex \textbf{input}: initial pose $\boldsymbol{v_{init}}$, No. of candidate viewpoints $n$
\Statex \textbf{output}: poseList   // all planned poses
\State $t \gets 0$;
\State $\boldsymbol{v} \gets \boldsymbol{v_{init}}$;
\State $planningFlag \gets True$;
\While {$t \leq N_{max}$ \textbf{and} $planningFlag$}
    \State $s_{occ}, P_{occ}, 
    \boldsymbol{f}, 
    D, Sems = sensing(\boldsymbol{v})$;
    \State $s_{pick} = s_{dis} * (1-s_{occ})$; 
    \State $\mathcal{M} = updateSemanticOctomap(D, Sems, \boldsymbol{v})$;
    \If {$s_{pick} > 0.9$}
        \State $planningFlag \gets False$;
        \State exit() // planning succeed;
    \EndIf
    \State $V_{vps} \gets uniformAdaptiveSampling(\boldsymbol{f}
    , P_{occ})$;
    \State $\boldsymbol{v_{nbv}} = \arg\max_{v \in V_{vp}}(score(\mathcal{M}, \boldsymbol{v}))$;
    \State Arm.move($\boldsymbol{v_{nbv}}$);
    
\EndWhile
\end{algorithmic}
\end{algorithm}
\vspace{-10pt}
\subsubsection{Viewpoint Planning Algorithm}
To find the next-best view, the planner first samples candidate viewpoints. Since the ideal picking points 
% for avocados 
lie along the picking ring, we define a sampling space $\mathcal{P}$, on a circle in 3D space with a 0.21 m radius (adjustable based on tree width), centered at $\boldsymbol{f}_{pos}$.
% Even when the avocado tree is fully positioned within the arm's workspace, 
% Since the rear portion of the avocado tree, further from the robotic arm, is difficult to reach, we restrict the sampling space to the arc of a 270-degree sector (this limitation can be removed if an aerial platform is used), and get two boundary points $p_{b}^{1}$ and $p_{b}^{2}$. 
% Since the rear portion of the avocado tree, further from the robotic arm, is difficult to reach,
% We restrict the sampling space to the arc of a 270 degree sector as the rear portion of the tree, further from the robotic arm, is difficult to reach (this limitation can be removed if an aerial platform is used). 
We constrain the sampling space to a 270\textdegree{} arc, as the rear portion of the tree is harder to reach with a robotic arm (this limitation can be removed with an aerial platform).
% Hence, we get 
This defines
two boundary points $p_{b}^{1}$ and $p_{b}^{2}$. 
\begin{figure}[!b]
% \begin{figure}[hpb]
    \vspace{-28pt}
    \centering
    \includegraphics[width=0.49\textwidth]{figs/vp_sampling_algo_4.png}
    \vspace{-16pt}
    \caption{A example for GS-NBV
    % viewpoint sampling 
    algorithm: The black dot represents the fixed arm base. The blue dot indicates the camera's current viewpoint, and the occluded fruit is discoverable within the camera's field of view, as shown by the blue lines. The green dot represents the estimated avocado position $\boldsymbol{f}_{pos}$. 
    % in the space from the current view. 
    The red circle, known as the picking ring, is defined by the sampling radius and the fruit pose 
    $\{\boldsymbol{f}_{pos}, \boldsymbol{f}_{axis}\}$. For simplicity here, assuming $\boldsymbol{f}_{pos}$ is fixed and $\boldsymbol{f}_{axis}$ always point outward perpendicular to the plane. The gray bars represent background objects in the environment (such as leaves or other tree parts), while the gray dots indicate boundary points. 
    Initially, the camera is positioned at $v_{iter1}$. In the $1^{st}$ iteration, four points on the picking ring (purple dots) are selected. $v_4$ is discarded (marked with a cross), and $v_1$ is selected as the next-best viewpoint (red dot). In the $2^{nd}$ iteration, the camera moves to $v_1$, 
    % and the fruit position $\boldsymbol{f}_{pos}$ and boundary points are updated. 
    the fruit pose and boundary points are updated. 
    Four new points are selected (orange dots). $v'_1$ and  $v'_3$ are discarded, and $v_3$ is chosen as the next-best viewpoint.}
    \label{fig:vp_sampling_algo}
    % \vspace{-24pt}
\end{figure}

Given the current 
% camera 
viewpoint $v_{iter1}$, we can get the obstacle points $ P_{occ}$ from the scene 
% and hence get two more boundary points $p_{occ}^{1}$ and $p_{occ}^2$. 
and hence get leftmost and rightmost obstacle points as boundary points $p_{occ}^{1}$ and $p_{occ}^2$. 
Thus, the sampling space further reduce to 
$\overset{\huge\frown}{p_{b}^{1}p_{occ}^{1}}\cup\overset{\huge\frown}{p_{occ}^{2}p_{b}^{2}}$. 
Since viewpoint planning is an iterative process and the sampling space on the picking ring progressively decreases, there is no need to sample a large number of viewpoints in each iteration. Thus, we uniformly selected four equidistant viewpoints: $v^1$, $v^2$, $v^3$ and $v^4$ from the updated sampling space $\mathcal{P}$.
% within the updated sampling space to determine four viewpoints: $v^1$, $v^2$, $v^3$ and $v^4$. 
Compared to extensive random viewpoint sampling~\cite{yi2024view,zaenker2021viewpoint}, this approach leverages the geometric properties of the avocado to reduce the subsequent computational costs of the Raycasting algorithm. Meanwhile it also ensures adequate spatial coverage of the avocado tree from various angles.
% maximal coverage of the avocado tree from various angles.
% Additionally, it avoids the issue of gradient-based methods becoming stuck in local minima.
Each viewpoint is represented by a seven-element vector, where the first three elements are position, and the last four elements are orientation in quaternion form. The quaternion is generated from the directional vector produced by the viewpoint's position relative to $\boldsymbol{f}_{pos}$.  For each viewpoint, we apply Raycasting algorithm and evaluate their utility scores. Viewpoints with utility scores below a certain threshold (set to 10) are removed.
% Additionally, if sampled viewpoints fall within a 0.1-meter radius of existing viewpoints or visited viewpoints, they are also excluded from the sampling space.
Additionally, if sampled viewpoints fall within a 0.1 m radius of previously sampled viewpoints, they are also removed from the sampling space.
The rationale here is to filter out those viewpoints that are too similar to previously selected ones, as they generally do not provide sufficient novel information. 
The concept is called \textit{viewpoint dissimilarity}, adapted from the NBV-SC approach~\cite{menon2023nbv}. 
The difference is that, in NBV-SC, 
they used a combination of angular and distance threshold whereas we only need a distance measure in our local planning setting.
% they used a combination of angular threshold and distance threshold  whereas we used a distance measure. 
% Specifically, we set this distance at 0.1 meters, which is the length of the camera box frame mounted on the arm end-effector, to ensure adequate spatial separation of viewpoints.
% they apply dissimilarity filter on angle threshold (chosen as 0.1), we apply the filter on distance measure of 0.2 m which is the 1.5 times of the length of the end-effector radius.
% Unlike the original method, which implements a dissimilarity filter based on an angular threshold of 0.1, our approach applies this filter using a distance measure to ensure distinct viewpoint selection.
% any sampled viewpoints located within a0.2 meters of existing viewpoints are also excluded from the sampling space to ensure distinct and effective coverage.
% , and the space within a 0.2 meters (\textcolor{red}{will change this number and explain later}) radius surrounding these points is also excluded from the sampling space. 
In Fig.~\ref{fig:vp_sampling_algo} (left), $v_4$ is discard due to low utility score in the first iteration and the update of bound point $p_b^2$ is shown in the second iteration.
The remaining candidate viewpoints, along with their associated utility scores, are ranked based on the total utility score and stored in a Viewpoint Queue, $V_{vps}$, in descending order. The viewpoint with the maximum utility was chosen as the next-best viewpoint: $\boldsymbol{v}_{\text{nbv}} = \arg\max_{\boldsymbol{v} \in V_{vps}} U_{\text{sem}}$. Here in Fig.~\ref{fig:vp_sampling_algo}, $\boldsymbol{v}_{\text{nbv}} = v_1$.
% with the highest total utility score, here $v_1$, is then selected as the next-best view (indicated by red dot in Fig.~\ref{fig:vp_sampling_algo}).
% Once the next-best viewpoint is selected, the arm motion planning is implemented by MoveIt~\cite{moveit} framework to handle singularities, self-collision avoidance, and trajectory execution. 
Once $\boldsymbol{v}_{\text{nbv}}$ is selected, the arm motion planning is implemented by MoveIt~\cite{moveit} framework. 
The first iteration ended up with camera moving to $v_1$.

As new observations are acquired, updates are made to both the fruit pose and the semantic OctoMap. From the updated fruit pose, a new picking ring is estimated. Subsequently, we project previous boundary points onto this new circle. This process ensures that the sampling space continually decreases, enhancing the efficiency of viewpoint sampling.
In the second iteration, two additional boundary points $p^3_{occ}$ and $p^4_{occ}$ are incorporated as the camera detects more obstacle points.
Hence the sampling space was updated to $\mathcal{P}$ = 
$\overset{\huge\frown}{p_{b}^{1}p_{occ}^{3 }}\cup 
\overset{\huge\frown}{p_{occ}^{4}p_{occ}^{1}} \cup \overset{\huge\frown}{p_{occ}^{2}p_{b}^{2}}$. 
Uniform equidistant sampling therefore yielded new viewpoints: $v'^1$, $v'^2$, $v'^3$ and $v'^4$. 
% The arc 
% $\overset{\huge\frown}{p_{b}^{1}p_{occ}^{3}}$ was discarded due to the distance between $p_b^1$ and $p_{occ}^{3}$ being less than 0.1 meters. 
However $v'^1$ and $v'^3$ were excluded because they fall within 0.1 m radius of 
previously sampled viewpoints. 
The newly selected viewpoints along with their utility scores, were saved to the Viewpoint Queue following a descending order.
\begin{figure}[!b]
\vspace{-20pt}
% \begin{figure}[hpb]
    % \vspace{-18pt}
    \centering
    \includegraphics[width=0.47\textwidth]{figs/sota_search_space2.png}
    % \includegraphics[width=0.45\textwidth]{figs/search_space_compare6_crop.png}
    \vspace{-2pt}
    \caption{Planner Search Space Comparison
 % between SCNBVP and GS-NBV
 }
    \label{fig:search_space_compare}
    % \vspace{-21pt}
\end{figure}Despite new iterations introducing additional observations and further exploring the map, only the motion costs part for viewpoints already in the queue were updated. The 
expected semantic information gains
will not be re-calculated. 
The reasons are threefold: 1) As Raycasting is a time-consuming process, not updating the expected semantic information gains can significantly save time and enhance efficiency; 2) It biases the planner towards selecting newer viewpoints, which are likely to provide more information; 3) Since the existing viewpoints remain unchanged and are thus underestimated, even if selected as the next-best view, they will not provide less information than previously anticipated. 
Therefore, $v^3$, a previously selected viewpoint with the highest utility in the queue was chosen as the next-best view in the second iteration.
In extreme cases, if the queue is empty, a new set of viewpoints will be re-sampled following the same rules outlined above.
This process continues iteratively until the fruit becomes pickable.
% \subsubsection{Viewpoint Evaluation}
% \subsubsection{Viewpoint Selection and Execution}
% From the Viewpoint Queue $V_{vps}$, the one with the maximum utility was chosen as the next-best viewpoint: $\boldsymbol{v}_{\text{nbv}} = \arg\max_{\boldsymbol{v} \in V_{vps}} U_{\text{sem}}
% $. Once the next-best viewpoint is selected, the arm motion planning is implemented by MoveIt~\cite{moveit} framework to handle singularities, self-collision avoidance, and trajectory execution. 


==> sections/4_1_nbv_algo_ori.tex <==
\subsection{Viewpoint Planning: GS-NBV}
The viewpoint planning algorithm is an iterative method consisting of 2 main steps: viewpoint sampling and evaluation.
% viewpoint evaluation. 
% Considering the distribution of avocado picking points, we proposed a \textbf{G}eometry-based, \textbf{S}emantics-aware \textbf{N}ext-\textbf{B}est \textbf{V}iew planning algorithm, termed GS-NBV. 
In this section, we first define the utility score to evaluate viewpoints, then elaborate our algorithm (Alg.~\ref{alg:mynbv}). 
% \vspace{-6pt}
\subsubsection{Viewpoint Utility Score}
\label{subsubsection:vp_eva}
The score consists of two components: the expected semantic information gain $G_{\text{sem}}(\boldsymbol{v})$ and the motion cost.
The semantic information $I_{\text{sem}}(x)$ of a voxel $x$ within the field of view of the viewpoint is used to measure uncertainty and calculated through Shannon's entropy: $I_{\text{sem}}(x) = -p_s(x) \log_2(p_s(x)) - (1 - p_s(x)) \log_2(1 - p_s(x))
$, where $p_s(x)$ is the 
semantic probability
that the voxel $x$ belonged to a certain non-background semantic class, ie. $c_s(x)\neq 1$ (our focus is on exploring objects of interest, rather than the surrounding space).
% the given viewpoint is calculated by .
$G_{\text{sem}}(\boldsymbol{v})$ quantifies the total expected semantic information gain from a given viewpoint $\boldsymbol{v}$~\cite{burusa2024gradient}. 
The equation is 
% the expected semantic information gain estimated
$G_{\text{sem}}(\boldsymbol{v}) = \sum_{x \in (X_v \cap V_{\text{ooi}})} T(x)I_{\text{sem}}(x)$. Here 
$X_v$ is the set of all voxels within the field of view, given viewpoint $\boldsymbol{v}$. 
$V_{ooi}$ is the set of ROI voxels. $T(x)$ is an indicator function which determines the visibility from a viewpoint $\boldsymbol{v}$ to a voxel $x$.
In our approach, $ T(x)$ is conceptualized differently from its usage in the GradientNBV framework~\cite{burusa2024gradient}. In GradientNBV, $ T(x)$ measures the accumulated transmittance along the ray up to point $x$, estimating the probability that the ray remains unobstructed. This allows for occluded semantic voxels within the field of view to still enhance information gain. Conversely, in our case, invisible semantic voxels do not contribute to information gain. If no semantic voxels are directly visible in the given viewpoint,  $G_{\text{sem}}(\boldsymbol{v})$ equals zero. 
This adjustment enhances the quality of candidate viewpoints by strictly enforcing visibility constraints.

In addition to expected semantic information gain, the distance from the current viewpoint was also considered when selecting the next best view. 
% due to the time cost associated with motion. 
Thus, the final utility score is obtaining by: 
$ U_{\text{sem}}(\boldsymbol{v})= G_{\text{sem}}(\boldsymbol{v}) \times e^{-\lambda d}
$, where $d$ is the Euclidean distance between the current viewpoint and the next potential viewpoint and $\lambda$ control the penalty on the motion cost. While most methods prioritize adjacent positions, in our local environment planning, motion cost is less critical. Moving to a distant position on the picking ring can intuitively enhance exploration of the target's surroundings. Hence, we set $\lambda$ to -1 to encourage distant movement.
% \vspace{-20pt}
\vspace{-20pt}
\begin{algorithm}
\caption{GS-NBV planning}
\label{alg:mynbv}
\begin{algorithmic}[1]
\Statex \textbf{input}: initial pose $\boldsymbol{v_{init}}$, No. of candidate viewpoints $n$
\Statex \textbf{output}: poseList   // all planned poses
\State $t \gets 0$;
\State $\boldsymbol{v} \gets \boldsymbol{v_{init}}$;
\State $planningFlag \gets True$;
\While {$t \leq N_{max}$ \textbf{and} $planningFlag$}
    \State $s_{occ}, P_{occ}, 
    \boldsymbol{f}, 
    D, Sems = sensing(\boldsymbol{v})$;
    \State $s_{pick} = s_{dis} * (1-s_{occ})$; 
    \State $\mathcal{M} = updateSemanticOctomap(D, Sems, \boldsymbol{v})$;
    \If {$s_{pick} > 0.9$}
        \State $planningFlag \gets False$;
        \State exit() // planning succeed;
    \EndIf
    \State $V_{vps} \gets uniformAdaptiveSampling(\boldsymbol{f}
    , P_{occ})$;
    \State $\boldsymbol{v_{nbv}} = \arg\max_{v \in V_{vp}}(score(\mathcal{M}, \boldsymbol{v}))$;
    \State Arm.move($\boldsymbol{v_{nbv}}$);
    
\EndWhile
\end{algorithmic}
\end{algorithm}
\vspace{-10pt}
\subsubsection{Viewpoint Planning Algorithm}
To find the next-best view, the planner needs to sample some candidate viewpoints first. Since the ideal picking points 
% for avocados 
located along the picking ring, we define a sampling space $\mathcal{P}$, on a circle in 3D space with a radius of 0.21 m (adjustable based on the width of the avocado tree), centered at $\boldsymbol{f}_{pos}$.
% Even when the avocado tree is fully positioned within the arm's workspace, 
% Since the rear portion of the avocado tree, further from the robotic arm, is difficult to reach, we restrict the sampling space to the arc of a 270-degree sector (this limitation can be removed if an aerial platform is used), and get two boundary points $p_{b}^{1}$ and $p_{b}^{2}$. 
% Since the rear portion of the avocado tree, further from the robotic arm, is difficult to reach,
We restrict the sampling space to the arc of a 270 degree sector as the rear portion of the tree, further from the robotic arm, is difficult to reach (this limitation can be removed if an aerial platform is used). Hence, we get two boundary points $p_{b}^{1}$ and $p_{b}^{2}$. 
\begin{figure}[!b]
% \begin{figure}[hpb]
    \vspace{-24pt}
    \centering
    \includegraphics[width=0.49\textwidth]{figs/vp_sampling_algo_4.png}
    \vspace{-16pt}
    \caption{A example for GS-NBV
    % viewpoint sampling 
    algorithm: The black dot represents the fixed arm base. The blue dot indicates the camera's current viewpoint, and the occluded fruit is discoverable within the camera's field of view, as shown by the blue lines. The green dot represents the estimated avocado position $\boldsymbol{f}_{pos}$. 
    % in the space from the current view. 
    The red circle, known as the picking ring, is defined by the sampling radius and the fruit pose 
    $\{\boldsymbol{f}_{pos}, \boldsymbol{f}_{axis}\}$. For simplicity here, assuming $\boldsymbol{f}_{pos}$ is fixed and $\boldsymbol{f}_{axis}$ always point outward perpendicular to the plane. The gray bars represent background objects in the environment (such as leaves or other tree parts), while the gray dots indicate boundary points. 
    Initially, the camera is positioned at $v_{iter1}$. In the $1^{st}$ iteration, four points on the picking ring (purple dots) are selected. $v_4$ is discarded (marked with a cross), and $v_1$ is selected as the next-best viewpoint (red dot). In the $2^{nd}$ iteration, the camera moves to $v_1$, 
    % and the fruit position $\boldsymbol{f}_{pos}$ and boundary points are updated. 
    the fruit pose and boundary points are updated. 
    Four new points are selected (orange dots). $v'_1$ and  $v'_3$ are discarded, and $v_3$ is chosen as the next-best viewpoint.}
    \label{fig:vp_sampling_algo}
    % \vspace{-24pt}
\end{figure}

Given the current camera viewpoint $v_{iter1}$, we can get the obstacle points $ P_{occ}$ from the scene 
% and hence get two more boundary points $p_{occ}^{1}$ and $p_{occ}^2$. 
and hence get leftmost and rightmost obstacle points as boundary points $p_{occ}^{1}$ and $p_{occ}^2$. 
Thus, the sampling space further reduce to 
$\overset{\huge\frown}{p_{b}^{1}p_{occ}^{1}}\cup\overset{\huge\frown}{p_{occ}^{2}p_{b}^{2}}$. 
Since viewpoint planning is an iterative process and the sampling space on the picking ring progressively decreases, there is no need to sample a large number of viewpoints in each iteration. Thus, we uniformly selected four equidistant viewpoints: $v^1$, $v^2$, $v^3$ and $v^4$ from the updated sampling space $\mathcal{P}$.
% within the updated sampling space to determine four viewpoints: $v^1$, $v^2$, $v^3$ and $v^4$. 
Compared to extensive random viewpoint sampling~\cite{yi2024view,zaenker2021viewpoint}, this approach leverages the geometric properties of the avocado to reduce the subsequent computational costs of the Raycasting algorithm. Meanwhile it also ensures adequate spatial coverage of the avocado tree from various angles.
% maximal coverage of the avocado tree from various angles.
% Additionally, it avoids the issue of gradient-based methods becoming stuck in local minima.
Each viewpoint is represented by a seven-element vector, where the first three elements are position, and the last four elements are orientation in quaternion form. The quaternion is generated from the directional vector produced by the viewpoint's position relative to $\boldsymbol{f}_{pos}$.  For each viewpoint, we apply Raycasting algorithm and evaluate their utility scores. Viewpoints with utility scores below a certain threshold (set to 10) are removed.
% Additionally, if sampled viewpoints fall within a 0.1-meter radius of existing viewpoints or visited viewpoints, they are also excluded from the sampling space.
Additionally, if sampled viewpoints fall within a 0.1 m radius of previously sampled viewpoints, they are also removed from the sampling space.
The rationale here is to filter out those viewpoints that are too similar to previously selected ones, as they generally do not provide sufficient novel information. 
The concept is called \textit{viewpoint dissimilarity}, adapted from the NBV-SC approach~\cite{menon2023nbv}. 
The difference is that, in NBV-SC, 
they used a combination of angular and distance threshold whereas we only need a distance measure in our local planning setting.
% they used a combination of angular threshold and distance threshold  whereas we used a distance measure. 
% Specifically, we set this distance at 0.1 meters, which is the length of the camera box frame mounted on the arm end-effector, to ensure adequate spatial separation of viewpoints.
% they apply dissimilarity filter on angle threshold (chosen as 0.1), we apply the filter on distance measure of 0.2 m which is the 1.5 times of the length of the end-effector radius.
% Unlike the original method, which implements a dissimilarity filter based on an angular threshold of 0.1, our approach applies this filter using a distance measure to ensure distinct viewpoint selection.
% any sampled viewpoints located within a0.2 meters of existing viewpoints are also excluded from the sampling space to ensure distinct and effective coverage.
% , and the space within a 0.2 meters (\textcolor{red}{will change this number and explain later}) radius surrounding these points is also excluded from the sampling space. 
In Fig.~\ref{fig:vp_sampling_algo} (left), $v_4$ is discard due to low utility score in the first iteration and the update of bound point $p_b^2$ is shown in the second iteration.
The remaining candidate viewpoints, along with their associated utility scores, are ranked based on the total utility score and stored in a Viewpoint Queue, $V_{vps}$, in descending order. The viewpoint with the maximum utility was chosen as the next-best viewpoint: $\boldsymbol{v}_{\text{nbv}} = \arg\max_{\boldsymbol{v} \in V_{vps}} U_{\text{sem}}$. Here in Fig.~\ref{fig:vp_sampling_algo}, $\boldsymbol{v}_{\text{nbv}} = v_1$.
% with the highest total utility score, here $v_1$, is then selected as the next-best view (indicated by red dot in Fig.~\ref{fig:vp_sampling_algo}).
% Once the next-best viewpoint is selected, the arm motion planning is implemented by MoveIt~\cite{moveit} framework to handle singularities, self-collision avoidance, and trajectory execution. 
Once $\boldsymbol{v}_{\text{nbv}}$ is selected, the arm motion planning is implemented by MoveIt~\cite{moveit} framework. 
The first iteration ended up with camera moving to $v_1$.

As new observations are acquired, updates are made to both the fruit pose and the semantic OctoMap. From the updated fruit pose, a new picking ring is estimated. Subsequently, we project previous boundary points onto this new circle. This process ensures that the sampling space continually decreases, enhancing the efficiency of viewpoint sampling.
In the second iteration, two additional boundary points $p^3_{occ}$ and $p^4_{occ}$ are incorporated as the camera detects more obstacle points.
Hence the sampling space was updated to $\mathcal{P}$ = 
$\overset{\huge\frown}{p_{b}^{1}p_{occ}^{3 }}\cup 
\overset{\huge\frown}{p_{occ}^{4}p_{occ}^{1}} \cup \overset{\huge\frown}{p_{occ}^{2}p_{b}^{2}}$. 
Uniform equidistant sampling therefore yielded new viewpoints: $v'^1$, $v'^2$, $v'^3$ and $v'^4$. 
% The arc 
% $\overset{\huge\frown}{p_{b}^{1}p_{occ}^{3}}$ was discarded due to the distance between $p_b^1$ and $p_{occ}^{3}$ being less than 0.1 meters. 
However $v'^1$ and $v'^3$ were excluded because they fall within 0.1 m radius of 
previously sampled viewpoints. 
The newly selected viewpoints along with their utility scores, were saved to the Viewpoint Queue following a descending order.
\begin{figure}[!b]
\vspace{-22pt}
% \begin{figure}[hpb]
    % \vspace{-18pt}
    \centering
    \includegraphics[width=0.47\textwidth]{figs/sota_search_space2.png}
    % \includegraphics[width=0.45\textwidth]{figs/search_space_compare6_crop.png}
    \vspace{-2pt}
    \caption{Planner Search Space Comparison
 % between SCNBVP and GS-NBV
 }
    \label{fig:search_space_compare}
    % \vspace{-21pt}
\end{figure}Despite new iterations introducing additional observations and further exploring the map, only the motion costs part for viewpoints already in the queue were updated. The 
expected semantic information gains
will not be re-calculated. 
The reasons are threefold: 1) As Raycasting is a time-consuming process, not updating the expected semantic information gains can significantly save time and enhance efficiency; 2) It biases the planner towards selecting newer viewpoints, which are likely to provide more information; 3) Since the existing viewpoints remain unchanged and are thus underestimated, even if selected as the next-best view, they will not provide less information than previously anticipated. 
Therefore, $v^3$, a previously selected viewpoint with the highest utility in the queue was chosen as the next-best view in the second iteration.
In extreme cases, if the queue is empty, a new set of viewpoints will be re-sampled following the same rules outlined above.
This process continues iteratively until the fruit becomes pickable.
% \subsubsection{Viewpoint Evaluation}
% \subsubsection{Viewpoint Selection and Execution}
% From the Viewpoint Queue $V_{vps}$, the one with the maximum utility was chosen as the next-best viewpoint: $\boldsymbol{v}_{\text{nbv}} = \arg\max_{\boldsymbol{v} \in V_{vps}} U_{\text{sem}}
% $. Once the next-best viewpoint is selected, the arm motion planning is implemented by MoveIt~\cite{moveit} framework to handle singularities, self-collision avoidance, and trajectory execution. 


==> sections/5_0_experiment.tex <==
\section{Experimentation and Results}
\subsection{Experiment setup}
\begin{table}[!t]
% \vspace{-16pt}
\centering
\caption{Planner Parameters Comparison}
\vspace{-6pt}
\label{table:sota_para_compare}
\begin{tabular}{lccc}
\toprule
\textbf{Parameter}&\textbf{GS-NBV}&\textbf{SC-NBVP} & \textbf{GNBV} \\
\midrule
RRT step size \(L\)                 & n.a        & 0.1m      & n.a                  \\
RRT max.nodes \(N_{\text{max}}\)    & n.a          & 10        & n.a                  \\
Min.gain \(g_{\text{zero}} L\)       & 10          & n.a       & n.a                  \\
Sampling dissimilarity     & 0.1m           & n.a       & n.a                \\
Number of candidate views \(n\)     & 4           & 4                  & 1        \\
% Degrees coefficient \(\lambda\)     & 0.01m        & 0.01m                    \\
% The movement cost coefficient
The motion cost coefficient \(\lambda\)     & -1        & 1           & n.a         \\
% Sampling spherical space radius \(R\)
Spherical sampling radius \(R\)
& n.a          & 0.1m             & n.a          \\
Octomap resolution \(r\)    &\multicolumn{3}{c}{0.003m}\\
Discrete point spacing \(\sigma\)   &\multicolumn{3}{c}{0.003m}  \\
% Camera Min. depth measure 
Camera minimum depth measure
&\multicolumn{3}{c}{0.03m}   \\
% Camera Max. depth measure 
Camera maximum depth measure 
&\multicolumn{3}{c}{0.72m}\\
Arm maximum reach&\multicolumn{3}{c}{0.60m}\\
\(R_{\text{min}}\) &0.21m &0.21m& n.a  \\
\(R_{\text{max}}\) &0.21m &0.21m & n.a \\
Octomap max-fusion coefficient &0.9 & n.a & 1.0 \\
Step size $\alpha$ &n.a& n.a & 0.65 \\
Picking score threshold &\multicolumn{3}{c}{0.90}\\
\bottomrule
\end{tabular}
\vspace{-24pt}
\end{table}
We assume a static and windless environment, where the movement of the robotic arm is accurate and does not have any impact on the pose of the avocado.
The experiments were conducted in two challenging simulated environments (Fig.~\ref{fig:init_end_plot}):
% We conducted the experiments in Gazeo simulation environment. 
an initial view with heavy occlusion (Group 1) and the same set up but with a board placed to the right side of the potted plant that completely blocks the visibility of viewpoints from the right side (Group 2). The avocado is placed vertically and occluded by leaves. 
% The initial views of planners are shown in Fig.~\ref{fig:init_end_plot}.

In the context of local planning, SC-NBVP~\cite{yi2024view} and GradientNBV (GNBV)~\cite{burusa2024gradient} represent the latest sampling-based and gradient-based work, and have shown superior performance in similar occlusion settings.
To evaluate our method, we compare it against SC-NBVP and GNBV. We optimized their parameters based on reported values and fine-tuned them for our setup (Table~\ref{table:sota_para_compare}). 
The ROI for all planners (including the fruit and peduncle) remained consistent, as shown by the green cuboid (Fig.~\ref{fig:algo_demo}). To accelerate SC-NBVP, we reduced its sampling space from 3D to 2D. The viewpoint sampling space for each planner is illustrated in Fig.~\ref{fig:search_space_compare}.

All the planners 
% The viewpoint planning algorithms 
were executed on a laptop equipped with an Intel i7-9750H CPU running at 2.60 GHz, 32 GB of RAM, and an NVIDIA RTX 2070 GPU with 8 GB of memory.  
Each planner was tested in 10 trials under identical conditions for each group independently and repeatedly. Each planning task will end either the fruit is \textit{pickable}
% when a picking point of the avocado is found (i.e. the fruit is \textit{pickable})
or when the maximum of 10 planning iterations are reached. 
\begin{figure}[!b]
% \begin{figure}[hpb]
    \vspace{-20pt}
    \centering
    \includegraphics[width=0.49\textwidth]{figs/init_end_sota_compare_brighter3.jpg}
    \vspace{-16pt}
    \caption{
    Comparison of the SC-NBVP and GNBV to our planner's inital view and the best final view selected from 10 trials in Group 1 (Top) and Group 2 (Bottom). 
    \textcolor{red}{might add one more group}
    % Best capture view compare Group 1 and 2 
    % (\textcolor{red}{add photos for each group)}
    }
    \label{fig:init_end_plot}
    % \vspace{-20pt}
\end{figure}
% \textcolor{red}{(Add more groups)}
% The purpose of the main experimental phase is two-fold: 1) to assess the overall avocado harvesting success rate, and 2) to determine XXX 
% In the context of local planning, SC-NBVP~\cite{yi2024view} and  GradientNBV(GNBV)~\cite{burusa2024gradient} are most recent work and have shown superior performance in a similiar occlusion settings.
% Several methods, such as AEP~\cite{selin2019efficient},  RVP~\cite{zaenker2021viewpoint} and SC-NBVP~\cite{yi2024view}, can be applied to this scenario. Among those, SC-NBVP~\cite{yi2024view}, a recent approach, has shown superior performance in a similar setting. Another recent work,
% GradientNBV(GNBV)~\cite{burusa2024gradient}, also XXX.
\subsection{Evaluation Metrics}
% The performance of our planner was validated in two scenarios:
% To evaluate our method, we compared it against SC-NBVP and GNBV.
% under two different occlusion scenarios. 
% Each method was tested in 10 trials under identical conditions for each group independently and repeatedly, and
The following metrics were used for evaluation:
% Each set of experiments started with avocado discoverable.
% All planners run independently and repeatedly
% 50 times and recorded metrics below:
\subsubsection{Successful rate}
The percentage of successful pickable viewpoints found out of 10 trials.
% \textcolor{red}{might need 30 trials each}

% The termination condition for each attempt is either reached the maximum 10 times planning or successfully identify a pickable viewpoint.
% The percentage of sucessful picking up in this 20 trials.
% Termination condition is: max 10 times planning or find the fruit pickable.
\subsubsection{Unoccluded rate} Defined by 1 - $s_{occ}$. A higher unoccluded rate increases the probability of successful fruit picking. A successful planning process requires the fruit to be fully discoverable with unoccluded rate exceeding a certain threshold (set to 0.9).
% A successful planning process entails a full discoverable fruit and 
\subsubsection{Fruit pose error} 
Measured by the average position error of the estimated avocado center from the ground truth position (set to [0.01, -0.36, 0.559]); and the average angular error of the estimated avocado axis from the ground truth axis (set to [0, 0, 1]) in Gazebo environment.
% Measured by the average position (and angular) error of the estimated avocado center (and axis) from the ground truth position (and axis) in Gazebo environment. The ground truth position (and axis) is set to [0.01, -0.36, 0.559] (and [0, 0, 1]).
% \subsubsection{Average ROI coverage} The percentage of voxels within the ROI that are explored by the camera.
% \subsubsection{Average viewpoint sampling}The mean count of sampled viewpoints per trial. It represents the computational cost of the planner since the ray casting algorithm is the most time consuming step. \textcolor{red}{The one time raycasting cost is 0.12 seconds for GNBV, and 0.06 seconds for our method and 0.2 seconds for SC-NBVP.} ~\ref{table:eva_nbv_time_compare}
% \subsubsection{Number of ray-tracing calls} \textcolor{red}{It indicated the com-putational cost of the view planners since the ray-tracingoperation was the most computationally expensive step. Thetime for one ray-tracing call was 0.06 seconds.}
% I am not pretty sure about this one, should I count this from successful picking.
% \subsubsection{Average planning instances}The average number of times the planner needs to adjust the camera pose to successfully pick the fruit.
\subsubsection{Number of planning iterations}The average number of planning iterations a planner required to complete the task. 
% \textcolor{red}{It represents the computational cost of the planner since the ray casting algorithm is the most time consuming step.}
It represents the computational cost of the planner since the ray casting algorithm is the most time consuming step.
% \textcolor{red}{
% The one time raycasting cost is 0.12 seconds for GNBV, and 0.06 seconds for our method and 0.2 seconds for SC-NBVP.} ~\ref{table:eva_nbv_time_compare
% }
\subsubsection{Time consumption} 
% The average time required by a specific planner to complete the task of finding picking points.
% The average time a planner required to complete the task.
The average time a planner required to complete a single viewpoint planning iteration.
% process.
% Generally, this indicator has high positive correlation with \textit{Number of planning iterations}. The more planning iterations required, the longer time it will take.
% \subsection{Simulation Experiment result and SOTA compare }
% The parameters were fine-tuned based avocado harvesting scenarios, and the adjusted parameters are presented in Tables~\ref{table:sota_para_compare} ).
% \begin{table}[h]
% \centering
% \caption{Planner Parameters Comparison}
% \label{table:sota_para_compare}
% \begin{tabular}{lccc}
% \toprule
% \textbf{Parameter}                  & \textbf{GS-NBV} & \textbf{SC-NBVP} & \textbf{GNBV} \\ \midrule
% RRT step size \(L\)                 & 0.1m         & 0.1m             & n.a          \\
% RRT max.nodes \(N_{\text{max}}\)    & 10           & 10               & n.a          \\
% Min.gain \(g_{\text{zero}} L\)       & 2.0          & n.a              & 2.0          \\
% Number of candidate views \(n\)     & 50           & 50               & 50           \\
% Degrees coefficient \(\lambda\)     & 0.01m        & 0.01m            & n.a          \\
% Sampling spherical space radius \(R\)& n.a          & 0.1m             & n.a          \\
% Octomap resolution \(r\)            & 0.005m       & 0.005m           & 0.005m       \\
% Discrete point spacing \(\sigma\)   & 0.0125m      & 0.0125m          & 0.0125m      \\
% \(R_{\text{min}}\)                  & 0.3m         & 0.3m             & 0.3m         \\
% \(R_{\text{max}}\)                  & 1m           & 1m               & 1m           \\ \bottomrule
% \end{tabular}
% \end{table}
% \subsection{Experiment Results and Analysis
% \textcolor{red}{-WIP-}
% }
\begin{table}[hb]
\vspace{-8pt}
\centering
\caption{Planner Time Consumption Comparison}
\vspace{-6pt}
\label{table:eva_nbv_time_compare}
\begin{tabular}{lccc}
\toprule
\textbf{Sub-process} [s]&\textbf{GS-NBV}&\textbf{SC-NBVP} & \textbf{GNBV} \\
\midrule
Viewpoints sampling&0.017        & 0.040     & \textbf{0}               \\
\midrule
Single raycasting call&0.199     & 0.645
% 1.310    
& 
 \multirow{2}{*}{\textbf{0.130}} \\
Viewpoints evaluation   &1.473       & 3.765   &             \\
\midrule
Compute next-best viewpoint   & \textbf{0.000}       & 0.072    & 0.328               \\
% Check trajectory exists &10.165&1.542&\textbf{ 0.054}\\
\midrule
NBV planning & 1.576 & 4.054     &\textbf{0.461}\\  
% NBV planning (w/o trajectory filter)& 1.576 & 4.054     &\textbf{0.461}\\  
% NBV planning (w/t trajectory filter)& 11.741 & 5.596    &\textbf{0.515}  \\
\bottomrule
\end{tabular}
% \vspace{-18pt}
\end{table}
\begin{table}[hb]
\vspace{-18pt}
\centering
\caption{Planners Performance Comparison}
\vspace{-6pt}
\label{table:success_rate}

% {\scriptsize % Begins a scope for smaller font size

\resizebox{0.49\textwidth}{!}{ % Shrinks table width to 85% of text width
\begin{tabular}{ccccc} 
\toprule
Metric & Group & GS-NBV & SC-NBVP& GNBV \\
\midrule
Success rate [\%] & \multirow{4}{*}{1} & \textbf{100\%} & 30\% & 60\% \\
% Time consumption [s] & & 34.89\smaller{$\pm10.55$} & 68.09\smaller{$\pm12.05$} & \textbf{25.87}\smaller{$\pm11.16$}\\
Fruit position error [m] & & \textbf{0.04$\pm0.00$}
 & 0.07$\pm0.08$ &0.15$\pm0.03$ \\
 Fruit axis error [$\circ$] &  & 22.63$\pm7.37$&\textbf{22.49}$\pm8.24$&30.00$\pm0.00$\\
% Avg. planning instances & & 88\% & 40\% \\
No. planning iterations& & \textbf{1.5} & 6&2.7\\
\addlinespace % Adds extra space between groups
% Success Rate [\%] & \multirow{4}{*}{2} & 100\% & 0\% &0\% \\
% Time consumption [s] &  & .74 & .04 &.00\\
% Fruit position error [m] &  & 0.016 & 0.223 \\
%  Fruit axis error [$\circ$] &  & 0.00\pm0.00&.09\pm.0&.82\pm.36\\
% % Avg. planning instances & & 88\% & 40\% \\
% No. viewpoints evaluated& & .4& .82 \\
% \midrule
% \addlinespace
Success Rate [\%] & \multirow{4}{*}{2} & \textbf{100\%} & 60\% & 50\% \\
% Time consumption [s] &  & 28.04\smaller{$\pm4.76$} & 59.79\smaller{$\pm15.32$} & \textbf{25.12}\smaller{$\pm7.67$}  \\
Fruit position error [m] &  &\textbf{0.02$\pm0.01$}&$0.09\pm0.09$&$0.13\pm0.06$\\
Fruit axis error [$\circ$] &  & $30.00\pm0.00$&\textbf{24.09$\pm9.90$}&$28.82\pm2.36$\\
% Fruit position error [m] &  &0.023\pm0.005&0.092\pm0.085&0.134\pm0.060\\
% Fruit axis error [$\circ$] &  & 30.000\pm0.000&24.094\pm9.901&28.819\pm2.362\\
% No. viewpoints evaluated& & 4.8& 22.5&2.6\\
No. planning iterations& & \textbf{1.2}& 4.5&2.6\\
\bottomrule
\end{tabular}
}
% } % Ends the scope for smaller font size
\vspace{-14pt}
\end{table}
\subsection{Results of the Planning Time Consumption and Analysis}

Table~\ref{table:eva_nbv_time_compare} shows the comparison of the planner's average time consumption in the viewpoint planning process. The NBV planning process is mainly implemented in 3 steps: viewpoints sampling, viewpoints evaluation and NBV computation.  
Bold font represents the best performance. 
In viewpoints sampling process, the time consumption of GNBV is zero as the gradient-based method does not sample viewpoints.
% In viewpoints sampling process, since GNBV is gradient-based method and does not require viewpoint sampling, thus the time consumption is zero. 
The one time raycasting cost is 0.199, 0.645, 0.130 seconds for our planner, SC-NBVP and GNBV respectively. 
% (Table~\ref{table:eva_nbv_time_compare}). 
Due to the more severe occlusion conditions in avocado growing environments compared to those of grapes, it is necessary to map the entire tree rather than only the ROI. This has led to much more time required for a single raycasting call in SC-NBVP than the time reported in their original work (0.136-0.162 seconds). Since the number of candidate views are 4, 4 and 1 for our planner, SC-NBVP and GNBV, the viewpoints evaluation process finally take 1.473, 3.765 and 0.130 seconds respectively.
In the NBV computation process, our method only select the viewpoint with highest utility, thus the time consumption is neglectable. SC-NBVP not only selects the viewpoint with highest utility but also computes the NBV using RRT algorithm, thereby resulting in a slightly longer computation time.
% compared to our method. 
GNBV needs to compute the gradient of the information gain function on the entire image, thereby resulting in the longest time consumption.
% To avoid collisions, we compute the feasible trajectory for each candidate view using MoveIt. Our method samples four scattered views that contain distant views from the current camera pose, resulting in longer computation times. In contrast, SC-NBVP and GNBV require feasible trajectory computation only for the final NBV, thereby significantly reducing computation time. Notably, in GNBV, the final NBV  is always near the current viewpoint, leading to the shortest trajectory computation time. 
% Without computing feasible trajectory (using an aerial platform), the whole NBV planning process takes 1.576, 4.054 and 0.461 seconds respectively.
The whole NBV planning process takes 1.576, 4.054 and 0.461 seconds respectively.

\subsection{Results of Planner Performance and Analysis}
% Table~\ref{table:success_rate} shows the comparison of the planner performance in each experiment groups. Bold font represents the best performance. 
Table~\ref{table:success_rate} presents a comparative analysis of planner performance across experiment groups, with the best results 
highlighted in bold.
% Except for the success rate, the other data was only calculated from successful attempts. 
% Data for metrics other than the success rate were derived solely from successful trials. 
Metrics other than the success rate were based only on successful trials.
% SC-NBVP showed improved success rate (from 30\% to 60\%) in the more challenging Group 2.
SC-NBVP's success rate improved from 30\% to 60\% in the more challenging Group 2.
% This is because in Group 2, the viewpoints sampled from the right side will produce high SC scores~\cite{yi2024view} and are less likely to be selected. 
This is because viewpoints from the right side in Group 2 generate high SC scores~\cite{yi2024view}, making them less likely to be selected.
This is equivalent to reducing the sampling space and 
hence will improve the 
% performance metrics such as
success rate and number of planning iterations. For the same reason, our planner also takes fewer iterations in the Group 2 (1.2 times) compared to the Group 1 (1.5 times). In both experimental groups, GNBV showed similar performance in success rate and number of planning iterations. In Fig.~\ref{fig:result_plot}, we separately plotted the average unoccluded rates curve for successful and failed attempts.
\begin{figure}[!t]
% \begin{figure}[hpb]
    % \vspace{-12pt}
    \centering
    \includegraphics[width=0.49\textwidth]{figs/sota_plot_compare_2exp_crop.png}
    \vspace{-16pt}
    \caption{
    % Results for the 
    Average unoccluded rate plot in two experiment groups. Solid and dashed lines indicate the results
    % average unoccluded rate
    from successful and 
    % attempts,
    % while dashed lines represent the same but from
    failed attempts respectively. The orange line at y = 0.9 represents the picking threshold. Once the fruit is fully discoverable, the planning process terminates, and the curve becomes flat.
    % SC-NBVP, GNBV, and our planner are indicated by green, blue, and red colors respectively.
    }
    \label{fig:result_plot}
    \vspace{-22pt}
\end{figure}
Due to the sampling randomness, \textit{SC-NBVP failure curve} fluctuates as the planning iterations  increase and does not converge. 
On the other hand, the \textit{GNBV failure curve} converges to local maxima and does not increase with more planning iterations.
% (especially in Group 1). 
In contrast, our method consistently achieved a 100\% success rate in both groups and identified a pickable view within two planning iterations.

Fig.~\ref{fig:init_end_plot} shows the qualitative result of the planners. The best captured final views of each planner are selected from 10 trials in both Group 1 and Group 2. In Group 1, all planners identified an ideal view. In Group 2, SC-NBVP still found an optimal view, while our planner's best final view was from below the fruit, and GNBV's from above.
However, in GNBV's final view,
it required the arm to navigate through a narrow gap between leaves and the board, posing a risk in real-world applications, especially with aerial platforms.
% In contrast, the GNBV failure line shows minimal change, especially in Group 1, due to being trapped in local maxima.
% Our method achieved a 100\% success rate in both experimental groups and identified a pickable view within two planning iterations.
% Therefore, we can see that the performance of sc-nbvp in group 2 is better than that in group 1 in terms of success rate and planning iterations (time consumption is an derivative metric from planning iterations) aspects.
% \vspace{-6pt}
\subsection{Results of Fruit Pose Estimation and Analysis}
% \vspace{-4pt}
Our method accurately estimates fruit position with the lowest mean error and standard deviation in both experiment groups due to the stable planner performance and 
equally consistent sampling distance on the picking ring.
% Our method can estimate the fruit position well with a low standard deviation. This is because our planner perform is stable always stay the same distance with the fruit; 
% SC-NBVP is random (either forward or backward)hence have high standard deviation. 
In contrast, the randomness in viewpoint sampling and RRT algorithm in SC-NBVP planner leads to relatively high mean position error and highest standard deviation.
GNBV has a smaller standard deviation than SC-NBVP, as it typically operates within a localized area. However, this also leads to the largest mean position error among three planners.
% GNBV std is smaller than SC-NBVP because it usually move on a local spot thus the std is small.

None of the planners estimate the fruit axis well in either group, but this does not hinder their ability to find a view for picking in highly occluded environments.
% All planners cannot estimate the axis of the fruit well in both groups, but this does not affect finding a view the fruit can be picked from highly occluded environment.


% Search space compare Fig.~\ref{fig:search_space_compare}
% \begin{table}[h]
% \centering
% \caption{Planner Performance Comparison}
% \label{table:success_rate}
% \begin{tabular}{cccc@{}} 
% \toprule
% Metric             & Group  & GS-NBV & SC-NBVP   \\ 
% \midrule
% Success rate [\%]  & 1 & 88\% & 40\% \\
% % \addlinespace
% Avg. total viewpoint evaluation time [s]&  1 & 57.72 & 111.98  \\
% Avg. fruit center distance error [m]  &  1 & 88\% & 40\% \\
% Avg. planning instances  &  1 & 88\% & 40\% \\
% \addlinespace % Adds extra space between groups
% Success Rate [\%]  &  2 & 82\% & 38\%  \\
% Avg. total viewpoint evaluation time [s]&  2 & 55.96 & 111.96  \\
% Avg. fruit center distance error [m]  &  2 & 88\% & 40\% \\
% \bottomrule
% \end{tabular}
% \end{table}


% \begin{table}[h]
% \centering
% \caption{Planner Performance Comparison}
% \label{table:success_rate}
% % \begin{tabular}{@{}p{4cm}cccc@{}} % Adjust column width here
% \begin{tabular}{ccccc@{}} % Adjust column width here
% \toprule
% Metric             & Group  & GS-NBV & SC-NBVP  & GNBV \\ 
% \midrule
% Success Rate [\%]  & Group 1 & 88\% & 40\% & 40\% \\
% Time Consumption [s] & Group 1 & 57.72 & 111.98 & 114.32 \\
% \addlinespace % Adds extra space between groups
% Success Rate [\%]  & Group 2 & 82\% & 38\% & 36\% \\
% Time Consumption [s] & Group 2 & 55.96 & 111.96 & 116.28 \\
% % \addlinespace % Adds extra space between groups
% % Success Rate [\%]  & Group 3 & 80\% & 38\% & 34\% \\
% % Time Consumption [s] & Group 3 & 55.65 & 110.31 & 121.32 \\
% \bottomrule
% \end{tabular}
% \end{table}


% \begin{table}[!b]
% \centering
% \caption{Planner Performance Comparison}
% \label{table:success_rate}
% \begin{tabular}{lcc}
% \toprule
% \textbf{Parameter}                  & \textbf{GS-NBV} & \textbf{SC-NBVP}  \\ \midrule
% RRT step size \(L\)                 & n.a        & 0.1m                       \\
% RRT max.nodes \(N_{\text{max}}\)    & n.a          & 10                         \\
% Min.gain \(g_{\text{zero}} L\)       & 10          & n.a                        \\
% Sampling dissimilarity \                  & 0.1m           & n.a                      \\
% Number of candidate views \(n\)     & 4           & 50                          \\
% % Degrees coefficient \(\lambda\)     & 0.01m        & 0.01m                    \\
% The movement cost coefficient \(\lambda\)     & -1        & 1                    \\
% Sampling spherical space radius \(R\)& n.a          & 0.1m                      \\
% Octomap resolution \(r\)            & 0.003m       & 0.003m                 \\
% Discrete point spacing \(\sigma\)   & 0.003m      & 0.003m              \\
% Camera minimum depth measure                   & 0.03m         & 0.03m                   \\
% Camera maximum depth measure                   & 0.72m           & 0.72m                      \\
% Arm maximum reach                  & 0.60m           & 0.60m                      \\
% \(R_{\text{min}}\) &0.21m &0.21m \\
% \(R_{\text{max}}\) &0.21m &0.26m \\
% \bottomrule
% \end{tabular}
% \end{table}

==> sections/void_6_0_conclusions.tex <==
\section{Conclusions and Future Research}
% \begin{table}[!t]
% \centering
% \caption{Planners Performance Comparison}
% \vspace{-6pt}
% \label{table:success_rate}
% {\scriptsize % Begins a scope for smaller font size
% \begin{tabular}{ccccc} 
% \toprule
% Metric & Group & GS-NBV & SC-NBVP& GNBV \\
% \midrule
% Success rate [\%] & \multirow{4}{*}{1} & \textbf{100\%} & 30\% & 60\% \\
% Time consumption [s] & & 34.89\smaller{$\pm10.55$} & 68.09\smaller{$\pm12.05$} & \textbf{25.87}\smaller{$\pm11.16$}\\
% Fruit position error [m] & & \textbf{0.04}\smaller{$\pm0.00$}
%  & 0.07\smaller{$\pm0.08$} &0.15\smaller{$\pm0.03$} \\
%  Fruit axis error [$\circ$] &  & 22.63\smaller{$\pm7.37$}&\textbf{22.49}\smaller{$\pm8.24$}&30.00\smaller{$\pm0.00$}\\
% % Avg. planning instances & & 88\% & 40\% \\
% No. planning iterations& & \textbf{1.5} & 6&2.7\\
% \addlinespace % Adds extra space between groups
% % Success Rate [\%] & \multirow{4}{*}{2} & 100\% & 0\% &0\% \\
% % Time consumption [s] &  & .74 & .04 &.00\\
% % Fruit position error [m] &  & 0.016 & 0.223 \\
% %  Fruit axis error [$\circ$] &  & 0.00\pm0.00&.09\pm.0&.82\pm.36\\
% % % Avg. planning instances & & 88\% & 40\% \\
% % No. viewpoints evaluated& & .4& .82 \\
% % \midrule
% % \addlinespace
% Success Rate [\%] & \multirow{4}{*}{2} & \textbf{100\%} & 60\% & 50\% \\
% Time consumption [s] &  & 28.04\smaller{$\pm4.76$} & 59.79\smaller{$\pm15.32$} & \textbf{25.12}\smaller{$\pm7.67$}  \\
% Fruit position error [m] &  &\textbf{0.02}\smaller{$\pm0.01$}&0.09\smaller{$\pm0.09$}&0.13\smaller{$\pm0.06$}\\
% Fruit axis error [$\circ$] &  & 30.00\smaller{$\pm0.00$}&\textbf{24.09}\smaller{$\pm9.90$}&28.82\smaller{$\pm2.36$}\\
% % Fruit position error [m] &  &0.023\pm0.005&0.092\pm0.085&0.134\pm0.060\\
% % Fruit axis error [$\circ$] &  & 30.000\pm0.000&24.094\pm9.901&28.819\pm2.362\\
% % No. viewpoints evaluated& & 4.8& 22.5&2.6\\
% No. planning iterations& & \textbf{1.2}& 4.5&2.6\\
% \bottomrule
% \end{tabular}
% } % Ends the scope for smaller font size
% \vspace{-20pt}
% \end{table}
%The avocado tree is a high-value crop (both in terms of fresh fruit and derivative products, such as oil) with growing global market demand~\cite{sommaruga2021avocado, duarte2016avocado, ayala2014avocado}. 
%However their cultivation in complex wild environments has hindered the automation of the harvesting processes.
%%% However, the automation of avocado harvesting remains underdeveloped due to their complex and wild growing environments. 
%While some progress has been made in designing the end-effector part~\cite{zhou2024design, liu2024vision, liu2024hierarchical}, the development of automated picking algorithms part is still missing. 
This paper presented a geometry-based, semantics-aware viewpoint planning algorithm for avocado harvesting under occlusion.
By defining the picking ring, we constrained the viewpoint search space to 1D, significantly improving the planning efficiency.
Additionally, we introduced the picking score metric to evaluate the selected viewpoints, ensuring the picking success rate. 
We evaluated our algorithm against state-of-the-art algorithms in two challenging simulated experiments. Our algorithm achieved a 100\% success rate with the fewest planning iterations. 
In contrast, the state-of-the-art algorithms achieved a maximum success rate of only 60\% in simulation, with significantly higher planning iterations. 
The results demonstrated
the effectiveness and robustness of our proposed approach.
% We demonstrated the effectiveness and robustness of our algorithm through two challenging simulated experiments and achieve 100\% success rate and smallest.
% designed to
% This paper presented a geometry-based, semantics-aware viewpoint planning-based algorithm designed to address this challenge, demonstrating its effectiveness through simulated experiments. 
The implementation of this work is expected to significantly increase harvesting efficiency for avocados. 
% By automating the picking process, it will relieve farmworkers from the labor-intensive tasks of climbing ladders and manually clipping fruits with clippers~\cite{mandemaker2006effects}, and enhancing the financial profitability for growers~\cite{fresh_avocado_market_us}.
Future work will focus on global planning strategies that pick multiple avocados from various trees within the orchard.






% Additionally, efforts will also be directed towards integrating the end-effector as in our earlier work for autonomous leaf cutting~\cite{campbell2022integrated}, deploying this system on an aerial platform to facilitate fully autonomous behavior and testing in local experimental farms to validate its effectiveness and efficiency in real-world agricultural settings.

% \textcolor{red}{TODO: related work; abstract; }
% \subsection{
% \begin{enumerate}
%     \item 
    % \item Finish up 
    % \item Fig.2 maybe find better avocado picture (with occlusion) first and say that the potted plant is simulate the avocado in real world 
    % \item \textit{Show sample space between SOTAs} draw the sample space of each method for compare. Extend Fig. 10 
    % \item \textit{Add tilt fruit experiments} 
    % \\ \textcolor{red}{Group 1\&2:} only avo partially visible (vertical axis)
    % \\ \textcolor{red}{Group 3\&4:} only avo partially visible (tilted axis)
    % \\ \textcolor{red}{Group 5\&6:} only ped partially visible (vertical axis)
    % \\ \textcolor{red}{Group 7\&8:} only ped partially visible (tilted axis)
    % \\ \textcolor{red}{Occlusion level:} Percentage of occlusion
    % \\ \textcolor{red}{Add this metric: Average ROI coverage:} The \% of ROI voxels that are explored by camera.
    % \item Finish writting: Experiment Results and Analysis
% \vspace{-6pt}
% \end{enumerate}


%%\\
% For automated fruit harvesting, identifying the picking point is essential. Unlike other fruits, picking avocados require specific viewpoints due to their unique harvesting challenges and highly unstructured growing environments. 
% In this work, we propose a novel geometry-based, semantics-aware viewpoint planning algorithm to address these issues. 
% We introduce the picking score metric to evaluate selected viewpoints and constrain the viewpoint search space to a 1D picking ring to improve planning efficiency. 

% Finally, we conducted comparative experiments on Kinova Jaco2 arm with two state-of-the-art methods. The results demonstrate a 100\% success rate in two challenging simulated environments, verifying the efficiency and robustness of our planning algorithm.
